Stability in Reaction Network Models via an Extension of the Next Generation Matrix Method

In this essay, we investigate some relations between Chemical Reaction Networks (CRN) and Mathematical Epidemiology (ME) and report on several pleasant surprises which we had simply by putting these two topics together. Firstly, we propose a definition of ME models as a subset of CRN models. Secondly, we review a fundamental stability result for boundary points, known in ME as the NGM method since it replaces the investigation of the Jacobian by that of a matrix whose origins lie in probability (the theory of branching processes). This important result seems to be little known outside of ME; even in ME, it has not been made clear before that the method gets sometimes the right answer, even though the conditions of the NGM theorem are not all satisfied. Thus, beyond the theorem, there is a heuristic approach, the validity conditions for which are not sufficiently understood. Thirdly, we show that some simple CRN models with absolute concentration robustness (ACR), are close qualitatively to simple ME models, in the sense that they have an unique disease free equilibrium, and a unique interior fixed point, and the latter enters the positive domain and becomes stable precisely when $R_0:=s_{dfe} \mathcal{R}=\frac{s_{dfe}}{s_e}>1.$ (where $s$ denotes the "ACR species"). Thus, for these "ME type models", a "relay phenomena" takes place: precisely when the DFE loses stability, a new fixed point enters the domain, and takes over. Last but not least, we offer in the associated GitHub repository https://github.com/adhalanay/epidemiology_crns a Mathematica package, Epid-CRN, which is addressed to researchers of both disciplines, and provide illustrative notebooks, which in particular solve a few minor open ME and CRN problems. Our package may also be used to study easy cases of analogue continuous time Markov chain (CTMC) ME and CRN models.

==> ACR.tex <==
\ssec{A bird's eye view on ACR \cite{ShiFei,karp2012complex,DexterGun,AliciaInv,tonello2018network,
PuenteJohn,joshi2024bifunctional}}
{A well-studied class of CRNs which frequently have boundary steady states are those with absolute concentration robustness.}
\beD
\label{d:ACR}
A mass action system $\mM = (\mS, \mC, \mR, k)$ is said to have:
\begin{enumerate}
\item
a \emph{robust ratio} between complexes $y$ and $y'$ if the ratio $\mathbf{x}^{y}/\mathbf{x}^{y'}$ takes the same value at every positive steady state $\mathbf{x} \in \mathbb{R}_{> 0 }^n$.
\item
\emph{absolute concentration robustness} in species $A$ if $x_A$ takes the same value at every positive steady state $\mathbf{x} \in \mathbb{R}_{> 0 }^n$. The value $x_A$ is called the \textit{ACR value} of $X_A$.
\end{enumerate}
\eeD
\noindent Note  that $x_A$ is independent of   the conservation constants and of the initial conditions, but this value does depend on the reaction constants $k$, and  that if two complexes $y$ and $y'$ have a robust ratio and differ only in a single species $A$, then ACR is guaranteed for $x_A$ \cite{ShiFei}.




ACR was first rigorously studied by Shinar and Feinberg~\cite{ShiFei} (interestingly, the simplest example they discuss is the  ME model with no demography known as SI, which they call ``toy model''). Recently, their sufficient conditions have been extended in ~\cite{joshi2024bifunctional}.

 \beXa The  \ME\ model SI, called ``toy model'' in \cite{ShiFei}, is:
$$\{
S+I \xrightarrow{k_1} 2I, ~ I \xrightarrow{k_2}S\}.$$  This system has exactly one positive steady state $(k_2/k_1, N_0 - k_2/k_1)$, where $N_0$ is the initial total population, and hence the network has  ACR in the first species $S$.
\eeXa

%Another  definition involving {\bf dynamic  ACR} was offered in~\cite{joshi-craciun,joshi-craciun-2}.

The first sufficient conditions for ACR, due to Shinar and Feinberg \cite{ShiFei}, have been restated in \cite{tonello2018network} as follows:
\beP
\label{thm:robustness_def0_def1}
Consider a  mass action system $\mM$.
\begin{enumerate}
\item
  If $\mM$ has a deficiency of zero and is weakly reversible,
  then it  has a robust ratio in each pair of complexes $y$ and $y'$ belonging to a common linkage class.
\item
  If $\mM$ has a deficiency of one and admits a positive steady state,
  then $\mM$ has a robust ratio in every pair of nonterminal complexes $y$ and $y'$ in $\N$.
\end{enumerate}
\eeP

\iffalse
 These conditions are also necessary for some classes of networks~\cite{meshkat-shiu}, and have been implemented in a Java-based system by~\cite{kuwahara2017acre}.

Recently, \cite{joshi2023prevalence} view ACR as a property opposite in some sense
to  multistationary, and show that asymptotically, as the expected number of  reactions tends to infinity, the following holds:


% ------------------
% SUMMARY TABLE
% ------------------
\begin{table}[ht]
\begin{center}
\begin{tabular}{l c c}
\hline
Expected number of reactions & Multistationary? & ACR? \\
\hline
% ------------------
Asymptotically greater than $1$, but less than $n^{2/3}$ & No & Yes \\
% ------------------
Asymptotically greater than $n$, but  less than $\frac{2}{17}n(\log(n)-c(n))$,
	& Yes & Yes \\
\hspace{.1in}  for some $c(n)\to\infty$ \\
% ------------------
Greater than $n(\log(n)+c(n) )$,   for some $c(n)\to\infty$
 & Yes & No \\
% ------------------
\hline
\end{tabular}
\end{center}
\caption{For random reaction networks, with $n$ species, %obtained under
generated by
a certain stochastic block model, this table lists ranges for the expected number of reactions, and whether -- with high probability -- such a network is multistationary or has ACR.}
\label{tab:summary-prevalence}
\end{table}%
% ------------------

\vspace{-0.1cm}

One sees from Table~\ref{tab:summary-prevalence} that the window for having both multi-stationarity and ACR is relatively small:
when the expected number of edges is asymptotically between $n$ and $\frac{2}{17}n\log(n)$.  The middle window only appears when there are thousands of species
\cite[Rem 4.14]{joshi2023prevalence}. ``We therefore expect that reaction networks with both multistationarity and ACR, in which the ACR species interacts nontrivially with other species, are rare and may require special structures or constructions".
\fi

ACR has also been analyzed using methods from computational
algebraic geometry~\cite{kaihnsa2024absolute, karp2012complex, beatriz,PuenteJohn}
(see also~\cite{case-study,CraStu}
for related works).
This is natural, in view of the fact that
 the ACR property is related to the ideal of the positive steady state locus~\cite{karp2012complex}.

\begin{proposition}[ACR and ideals] \label{prop:ideal}
A mass-action system $( \mM, \kappa)$ has ACR in species $X_i$
if and only if
$x_i - \alpha$, for some $\alpha >0$, is in the ideal of the positive steady state locus of $(\mM,\kappa)$.
\end{proposition}

  Conservative ACR systems  have always boundary steady states, owing to the following result.

\beT If a biochemical system admits: 1) an ACR species $Y,$ with ACR value $y^*$, and 2) a positive conservation law,  then  it must have a unique
fixed point $x^*$   on the boundary of the positive orthant, of minimal support, whose support includes the species $Y$.

\eeT

\prf
 Let $X_j$ denote the ACR species and $x_j^*$ denote the ACR value. Since the system has a positive conservation law, we have
\begin{equation}
\label{cons}
\sum_{i=1}^n c_i x_i = x_{tot}\in \mR_+,
\end{equation}
where $c_i > 0$ for all $i = 1, \ldots, n$.  At the positive steady state we can rearrange this to
\[0 < \mathop{\sum_{i=1}^n}_{i\not=j} c_i x_i = x_{tot} - c_j x_j^* < 0\]
which is a contradiction if  $x_{tot}$ is chosen sufficiently small, \satg\ $x_{tot} - c_j x_j^* < 0$. Consequently, there is no positive steady state for such values of $x_{tot}$.
Since the invariant space is a subset of the intersection of \eqref{cons} with the positive orthant, it is compact and therefore must contain a steady state. It follows that this
steady state must be on the boundary of the positive orthant.






==> EnvZ.tex <==
%\subsection{Computing $R_0$  for several representations of  the Escherichia coli EnvZ-OmpR osmolarity regulator}

\subsection{Examples of  Escherichia coli EnvZ-OmpR models, with ACR species Yp, where  \eqr{R0fr} holds}\lab{s:EnvZs}

\subsubsection{A  (5,4,3,1) subnetwork of   EnvZ-OmpR : EnvZ.nb}\lab{s:EnvZ}

This section considers a simplified EnvZ-OmpR  system represented in \cref{f:EnvZgr}
%\begin{equation}
%\label{envzompr}
%\begin{tikzcd}
%X  \arrow[r,"k_1"] & X_t  \arrow[r,"k_2"] & X_p \\[-0.1in]
%X_p + Y \arrow[r,"k_3"] & X  + Y_p \\[-0.1in]
%X_t  + Y_p \arrow[r,"k_4"] & X_t  + Y
%\end{tikzcd}
%\end{equation}
with \sm:
\bea \left(
\begin{array}{cccc}
 -1 & 0 & 1 & 0 \\
 1 & -1 & 0 & 0 \\
 0 & 1 & -1 & 0 \\
 0 & 0 & -1 & 1 \\
 0 & 0 & 1 & -1 \\
\end{array}
\right),\eea rank $3$,  \defi\ $1=7-3-3$.

%EnvZ.nb
\figu{EnvZgr}{The FHJ graph of the ``EnvZ-OmpR network" with $4$ reactions and the deficiency $\de=7-3-3=1$.}{1} 


 The corresponding system of ordinary differential equations is:
\begin{equation}
\label{de}
\frac{d}{dt} \left( \begin{array}{c} X \\ X_t \\ X_p \\ Y \\ Y_p \end{array} \right) = \left( \begin{array}{c} -k_1 X  + k_3 X_p Y \\ k_1 X  - k_2 X_t \\ k_2 X_t  - k_3 X_p Y \\ -k_3 X_p Y + k_4 X_t  Y_p \\ k_3 X_p Y - k_4 X_t  Y_p \end{array} \right)
\end{equation}
%\begin{equation}
%\label{de}
%\left\{ \begin{aligned}
%X' & = -k_1 X  + k_3 X_p Y \\
%X_t ' & = k_1 X  - k_2 X_t \\
%X_p' & = k_2 X_t  - k_3 X_p Y \\
%Y' & = -k_3 X_p Y + k_4 X_t  Y_p \\
%Y_p' & = k_3 X_p Y - k_4 X_t  Y_p
%\end{aligned} \right.
%\end{equation}
(to simplify the notation, we  have abbreviated, as customary,  EnvZ by X, and OmpR by Y). This example  satisfies the sufficient \cite{ShiFei}
ACR conditions,  since it  has deficiency one, and two non-terminal complexes
$X_t, X_t+Y_p$ (see \cref{f:EnvZgr}),
which
  differ in the single species $Y_p$ (which must therefore be  the ACR species).
  
 %\figu{EnvZOc}{Flow chart corresponding to the system \eqr{de}. }{1}
  
  
\BEN \im Our first step is the determination of the flux cone,  generated here by  $\left(
\begin{array}{c}
 1 \\
 1 \\
 1 \\
 1 \\
\end{array}
\right)$, and of  the conservation laws $x_{tot} = X  + X_t  + X_p, y_{tot} = Y + Y_p$, (total EnvZ and total OmpR, \resp). Both are found using our script ``cons'', which simply solves the linear kernel equations under non-negativity constraints on the variables.

 \im The second step is trying to get information on the non-negative fixed points. In simple examples like the ones discussed in this paper, 
 \lstinline[language=Mathematica]{Solve[RHS==0,var]} (the imperfect, quicker version of Reduce) finds quickly all the steady states. In this example, it finds  two boundary ones,  with two common invading components $ X =X_ t = 0$. Under this condition, the steady points must still have $ X_p Y =0$. The first possibility is incompatible with the positivity
of the first conservation, and the second,  $ Y= 0$, yields the DFE $$X  =  X_t  =0=Y,  X_p  =x_{tot},  Y_p =y_{tot},$$
with resident species set $\{ X_p, Y_p\}$.

\beR When Solve doesn't finish in reasonable time, it can be replaced by a search for boundary points, which are in fact typically easier to find (even when interior points aren't). %as is the custom
\eeR


 Solve identifies here also a third fixed point with  all \coords\ positive, parametrized by $x  ^*,x_p  ^*$,  \satg:
\[x_t  ^*=\frac{k_1 x  ^*}{k_2}, y  ^*= \frac{k_1 x  ^*}{k_3 x_p  ^*}, y_p ^*=\frac{k_2}{k_4} \leq y_{tot},\]
the last component $y_p ^*$ being the ACR species.
Note the last natural inequality, which turns out here to imply  both uniqueness of the interior point within each invariant set, parametrized  by $x_{tot}, y_{tot}$,  (so, finally, this is an example of trivial ACR), and stability, as shown next.

\im The next  step is trying to apply the NGM theorem (and even when it does not apply,  we get useful information by applying it formally -- examples below for further remarks).

The NGM  approach projects first the ODE on a group of ``infectious/invading'' species,  selected among the species which are zero at a boundary steady state (they are the ones which will increase/invade, if an outbreak occurs).


Here, the set of all infectious species is $\{ X, X_t , Y \}$ (see first step), and  the RHS of the
infection equations is
\[RHS_i=\bep k_3 Y X_p-k_1 X\\k_1 X-k_2 X_t\\k_4 Y_p X_t-k_3 Y X_p\eep=\mF-\mV:=\bep
 k_3 Y X_p\\0\\k_4 Y_p X_t\eep-\bep k_1 X\\k_2 X_t-k_1 X\\k_3 Y X_p\eep\]
 Here, $RHS_i$ has been split into the part of ``new infections" $\mF$
containing  all the interactions with positive sign \cite{AABJ}, and  the rest, denoted by $-\mV$, with the purpose of replacing the study of the spectrum of Jacobian $J_i$ \eqr{jI}
by that of the ``next generation matrix" \eqr{K}.

 Since the sum of the rows of $\mV$,  $k_2 X_t+k_3 Y X_p$ is unconditionally positive, and the other conditions of \cite{Van,Van08} also apply, we may apply the NGM theorem.

The derivative of $RHS_i$ \wrt\ the infection variables is:
\begin{gather}\label{jI} \nonumber J_i=\left(
\begin{array}{ccc}
 -k_1 & 0 & k_3 X_p   \\
 k_1 & -k_2 & 0 \\
 0 & k_4 Y_p   & -k_3 X_p   \\
\end{array}
\right)=F-V=\left(
\begin{array}{ccc}
 0 & 0 & k_3 X_p   \\
 0 & 0 & 0 \\
 0 & k_4 Y_p   & 0 \\
\end{array}
\right)-\\
\left(
\begin{array}{ccc}
 k_1 & 0 & 0 \\
 -k_1 & k_2 & 0 \\
 0 & 0 &
 k_3 X_p   \\
\end{array}
\right) \Lra
\end{gather}

\be{K} K = FV^{-1} = \left( \begin{array}{ccc}
0 & 0 & 1 \\
0 & 0 & 0 \\
\displaystyle{\frac{k_4 y_{tot}}{k_2}} & \displaystyle{\frac{k_4 y_{tot}}{k_2}} & 0
\end{array}
\right)
\ee
where the resident species $X_p, Y_p$ are evaluated
at the ``disease-free state" (with $X  = X_t = Y = 0$),
i.e. $X_p = x_{tot}, Y_p = y_{tot}$ (this is implemented in our script NGM).
\im The next step consists in attempting to
factor  the \ch\  of $K$, and in removing ``stable factors" (i.e. factors which may not have \eig s with positive real part). It seems, at least for the ACR models \satg\ the \cite{ShiFei} conditions discussed in this chapter,   that the \ch\ of $K$ factors more often than that of $J_i$.

 In our current example, the 3rd degree \ch\ of $K$ is $ch(u)=u (k_2 u^2-k_4 Y_p)$. After removing the factor $u$,    the remaining second degree polynomial has symmetric roots, the positive one being
$$R_0=\sqrt{\frac{k_4 y_{tot}}{k_2}}=\sqrt{\frac{ y_{tot}}{y_p  ^*}}.$$


Finally, the condition  $R_0 > 1$ under which the stability of the boundary  disease-free steady state is lost is precisely
\be{ACRi}y_{tot} > \frac{k_2}{k_4}=y_p^*.\ee

\beR When the  \ch\ has higher degree, we may also apply,  alternatively, the RH criteria to the shifted polynomial $p(x)=ch(x+1)$. In our current example,
the shifted second degree polynomial is $k_2 x^2+2 k_2 x+k_2-k_4 Y_p$, and RH recovers
the condition $k_2-k_4 Y_p\ge 0$. The computational advantage of this approach is that the single condition $R_0 \leq 1,$  with $R_0$ which may be the root of a high order polynomial, may be replaced by several RH conditions. These may be simpler sometimes, as will be illustrated in the   examples below.
\eeR

\EEN

\beR Here, $R_0$ may be  obtained  also using the Jacobian $J_i$ (whose \ch\ does not factor).
Indeed, the non-zero roots $\l$ of this \ch\ turn out to \saty\
$$\left(\lambda/k_1 +1\right) \left(\lambda/k_2+1\right) \left(\lambda/(k_3 X_p  )+1 \right)=  k_4  Y_p  /k_2,$$
and an eye inspection (or \Ma) checks that a crossing of $0$ by $\l$ occurs  iff $R_0=1$; however, the computation which uses the NGM matrix $K$ is easier, possibly due to the larger number of $0$'s, as compared to using the reduced Jacobian $J_i$, which does not factor.
\eeR



\beR \lab{r:Env}  The stability of the endemic point (when it exists) may also be
quickly checked, via:
\begin{lstlisting}
Reduce[Append[Join[ct, Thread[co > 0]], H3=co_2 co_3-co_1 co_4 > 0]]
\end{lstlisting}
where  ct denote all the positivity conditions (parameters and variables),
co denote the coefficients of the Jacobian reduced to three dimensions by dividing by $\l^2$, and H3 is the third  Hurwitz determinant.

  In conclusion,
we have shown that for the simplified EnvZ-OmpR that a typical scenario for ME models \cite{Diek,Van,Van08} holds: for $R_0 <1 \Eq y_{tot} < y_p^*$ the DFE is locally stable, and for $R_0 \ge 1 \Eq y_{tot} \ge y_p^*, $ the second endemic point enters the positivity domain and takes over the ``stability relay" from the DFE.
\eeR







==> EnvZCap.tex <==
%\subsubsection{A (8,9,,) version of  EnvZ-OmpR studied by \cite{AliciaMessi}}
%The CRN
%${\bc X <-> X_t-> X_p,\\
    %  X_p+Y<-> XpY -> X+Y_p,\\
     % X_t+Y_p<-> XtYp -> X_t+Y\ec}$

\subsubsection{A (8,11,6,1) subnetwork of  EnvZ-OmpR \cite{cappelletti2020hidden}: EnvZCap.nb}\lab{s:EnvZCap}

 We present  here  a subnetwork of the  EnvZ-OmpR model, which was studied by  \cite{cappelletti2020hidden}, and which  is obtained by ignoring the last line in the more general EnvZ-OmpR model  studied in \cite{ShiFei,karp2012complex} (see also \eqr{EJ} below):
%\be{Cap}
%      \begin{tikzcd}
%X_d \arrow[r,yshift=+0.5ex,"k_1"] & X \arrow[l,yshift=-0.5ex,"k_2"] \arrow[r,yshift=+0.5ex,"k_3"]& X_t \arrow[l,yshift=-0.5ex,"k_4"] \arrow[r,"k_5"]& X_p\\[-0.1in]
%X_p + Y \arrow[r,yshift=+0.5ex,"k_6"] & XpY \arrow[l,yshift=-0.5ex,"k_7"] \arrow[r,yshift=+0.5ex,"k_8"]& X + Y_p & \\
%[-0.1in]
%X_d + Y_p \arrow[r,yshift=+0.5ex,"k_9"] & XdYp \arrow[l,yshift=-0.5ex,"k_{10}"] \arrow[r,yshift=+0.5ex,"k_{11}"]& X_d + Y &
%      \end{tikzcd}
%%\schemestart
%%EnvZ-D  \arrow(1--2){<=>[*0{$k_1$}][*0{$k_2 $}]} EnvZ \arrow(@2--3){<=>[*0{$k_3 $}][*0{$k_4$}]} EnvZ-T \arrow(@3--4){->[*0{$k_5$}]} EnvZ-P
%%\arrow(@1.south east--.north east){0}[-90,.50]
%%EnvZ-P \+ OmpR \arrow(5--6){<=>[*0{$k_6$}][*0{$k_7$}]} EnvZ-OmpR-P \arrow(@6--7){->[*0{$k_8$}]} EnvZ \+ OmpR-P
%%\arrow(@5.south east--.north east){0}[-90,.50]
%%EnvZ-D \+ OmpR-P \arrow(8--9){<=>[*0{$k_9$}][*0{$k_{10}$}]} EnvZ-OmpR-D-P \arrow(@9--10){->[*0{$k_{11}$}]} EnvZ-D \+ OmpR
% %\schemestop
%\ee

%EnvZCap.nb
\figu{EnvZCapgr}{The FHJ graph of the ``(8,11,6,1) subnetwork of EnvZ-OmpR " with $11$ reactions and the deficiency $\de=10-3-6=1$.}{1}

\beR A) As in section \ref{s:EnvZs}, we interpret EnvZ as X, and OmpR as Y.  Note  that
alternations of capital and small letters following each other, like in XdYp, will denote \fno\ a single variable, while the same juxtaposition, but using sub-indices, will denote a product $X_d Y_p=X_d *Y_p$.

B) The conditions of \cite{ShiFei} identify OmpR$=Y_p$ as an ACR species.
\eeR


Ordering  the species (and the complexes) according to their appearance order yields the ODE: \beq &&\lab{ODEC}\frac{d}{dt} \bep X_d\\
 X\\
  X_t\\
   X_p\\
   Y\\
 XpY\\
  Y_p\\
   XdYp\eep=
   \bep-X_d \left(k_9 Y_p+k_1\right)+k_2 X+
   \left(k_{10}+k_{11}\right) {XdYp}
   \\k_1 X_d+k_4 X_t-X \left(k_2+k_3\right) +k_8 {XpY}\\k_3 X-\left(k_4+k_5\right) X_t\\-k_6 Y X_p+k_5 X_t+k_7 {XpY}\\-k_6 Y X_p+k_{11} {XdYp}+k_7 {XpY}\\k_6 Y X_p-\left(k_7+k_8\right) {XpY}\\-k_9 X_d Y_p+k_{10} {XdYp}+k_8 {XpY}
   \\k_9 X_d Y_p-\left(k_{10}+k_{11}\right) {XdYp}\eep\\&&=\left(
\begin{array}{c}
 0 \\
 0 \\
 0 \\
 0 \\
 0 \\
 k_6 Y X_p \\
 0 \\
 k_9 X_d Y_p \\
\end{array}
\right)-
\left(
\begin{array}{c}
 k_9 X_d Y_p+k_1 X_d-k_2 X -\left(k_{10}+k_{11}\right) {XdYp}\\
 -k_1 X_d-k_4 X_t+(k_2+k_3) X -k_8 {XpY}\\
 \left(k_4+k_5\right) X_t-k_3 X \\
 k_6 Y X_p-k_5 X_t-k_7 {XpY} \\
 k_6 Y X_p-k_{11} {XdYp}-k_7 {XpY} \\
 (k_8 +k_7) {XpY} \\
 k_9 X_d Y_p-k_{10} {XdYp}-k_8 {XpY} \\
  \left(k_{10}+k_{11}\right){XdYp} \\
\end{array}
\right).\eeq

%\figu{EnvZCapc}{Flow chart corresponding to the ODE \eqr{ODEC} where the sum of the RHS yields $-k_9 X_d Y_p-k_6 Y X_p+\left(k_{10}+k_{11}\right) XdYp+\left(k_7+k_8\right) XpY$, and the node $0$ corresponds to the \blue{exterior outputs and inputs. } }{1}

The system \eqr{ODEC} admits the following DFE:
$$ \pr{X=0,X_d=0,X_t=0,Y=0,XpY=0,XdYp=0}. $$

After removing  the fourth and seventh row in $\mV$, which correspond to resident variables, we find that the sum of the rows in
$$\mV=\left(
\begin{array}{c}
 k_9 X_d Y_p+k_1 X_d-k_2 X -\left(k_{10}+k_{11}\right) {XdYp}\\
 -k_1 X_d-k_4 X_t+(k_2+k_3) X -k_8 {XpY}\\
 \left(k_4+k_5\right) X_t-k_3 X \\

 k_6 Y X_p-k_{11} {XdYp}-k_7 {XpY} \\
 (k_8 +k_7) {XpY} \\

  \left(k_{10}+k_{11}\right){XdYp} \\
\end{array}
\right),$$ given by  $k_9 X_d Y_p
 +k_5 X_t+
k_6 Y X_p
 $ is unconditionally positive, and  we may apply the NGM theorem.

\BEN \im
It can be checked that, for that example, $rank(\Gamma)=6$ and the deficiency is
$\delta=m-rank(\Gamma)-\ell=10-6-3=1.$
The CRN is conservative, and the conservations are generated by:
\begin{equation}\label{eq:cons_envz}
\left\{X_d+X_p+X_t+X+{XdYp}+{XpY},Y_p+{XdYp}+{XpY}+Y\right\}
\end{equation}
(corresponding to the fact that the total mass of the chemical species containing some form of EnvZ is conserved, as well as the total mass of the chemical species containing some form of OmpR). The cone of positive fluxes has dimension 4.

 \im \Ma\ yields the following rational parametrization (RAP) parametrized by $X_d,X_p$, which is computed   using Solve[RHS==0] without specifying the ``var":
\be{SCap}\bc X= \frac{k_1 X_d}{k_2},X_t= \frac{k_1 k_3 X_d}{k_2 \left(k_4+k_5\right)},\\Y= \frac{k_1 k_3 k_5 \left(k_7+k_8\right) X_d}{k_2 \left(k_4+k_5\right) k_6 k_8 X_p},\text{XpY}= \frac{k_1 k_3 k_5 X_d}{k_2 \left(k_4+k_5\right) k_8},\\Y_p^*= \frac{k_1 \left(k_{10}+k_{11}\right) k_3 k_5}{k_{11} k_2 \left(k_4+k_5\right) k_9},\text{XdYp}= \frac{k_1 k_3 k_5 X_d}{k_{11} k_2 \left(k_4+k_5\right)}\ec\ee




\im  The NGM approach, applied to the 6D projection on the DFE coordinates, yields 4 eigenvalues equal to 0, and two satisfying a quadratic equation (again, the \ch\ of $K$ factors, while that of $J_i$ doesn't).
After shifting the polynomial, as explained in point 4. of the previous section,
we obtain a polynomial whose free coefficient at the DFE is
$$co_1=k_8 \left(k_1 \left(k_{10}+k_{11}\right) k_3 k_5-k_{11} k_2 \left(k_4+k_5\right) k_9 y_{tot}\right),$$
and the other two coefficients are positive.

 In conclusion, the stability domain of the DFE, obtained from
  $co_1>0$, is:
\be{ECint} y_{tot} \leq \frac{k_1 \left(k_{10}+k_{11}\right) k_3 k_5}{k_{11} k_2 \left(k_4+k_5\right) k_9} \Eq R_0:=\fr{y_{tot}}{Y_P^*}\leq 1. \ee

\EEN


==> EnvZJ.tex <==
\subsection{The DFE stability domain for the (9,14,7,2)   EnvZ-OmpR \cite{ShiFei,karp2012complex,JMP} does not \saty\ \eqr{R0fr}: EnvZJ.nb}\lab{s:EnvJ}
The original EnvZ-OmpR  first studied in \cite{ShiFei} was subsequently simplified in
\cite[Ex 18]{JMP}:
\be{EJ}
      \begin{tikzcd}
X_d \arrow[r,yshift=+0.5ex,"k_1"] & X \arrow[l,yshift=-0.5ex,"k_2"] \arrow[r,yshift=+0.5ex,"k_3"]& X_t \arrow[l,yshift=-0.5ex,"k_4"] \arrow[r,"k_5"]& X_p\\[-0.1in]
X_p + Y \arrow[r,yshift=+0.5ex,"k_6"] & XpY \arrow[l,yshift=-0.5ex,"k_7"] \arrow[r,yshift=+0.5ex,"k_8"]& X + Y_p & \\
[-0.1in]
X_d + Y_p \arrow[r,yshift=+0.5ex,"k_9"] & XdYp \arrow[l,yshift=-0.5ex,"k_{10}"] \arrow[r,yshift=+0.5ex,"k_{11}"]& X_d + Y &  \\[-0.1in]
X_t + Y_p \arrow[r,yshift=+0.5ex,"k_{12}"] & XtYp \arrow[l,yshift=-0.5ex,"k_{13}"] \arrow[r,yshift=+0.5ex,"k_{14}"]& X_t + Y &
      \end{tikzcd}
\ee
 %where $X_d =  {EnvZ-D}$, $X =  {EnvZ}$, $X_t =  {EnvZ-T}$, $X_p =  {EnvZ-P}$, $Y = {OmpR}$, $XpY =  {EnvZ-OmpR-P}$, $Y_p =  {OmpR-P}$, $XdYp =  {EnvZ-OmpR-D-P}$ and $XtYp =  {EnvZ-OmpR-T-P}$.
 The corresponding system of ordinary differential equations is
\begin{equation}
\label{EnvZOmpRDE}
%\left\{
%\begin{aligned}
%X_d' & =  -k_9 X_d Y_p - k_1 X_d + k_2 X + (k_{10} + k_{11}) XdYp \\
%X' & =  k_1 X_d - (k_2 + k_3) X + k_4 X_t + k_8 XpY\\
%X_t' & =  k_3 X - (k_4 + k_5) X_t - k_12 X_t Y_p + (k_{13} + k_{14}) XtYp \\
%X_p' & =  -k_6 X_p Y + k_5 X_t + k_7 XpY\\
%Y' & =  -k_6 X_p Y + k_{11} XdYp + k_{14} XtYp + k_7 XpY\\
%XpY' & =  k_6 X_p Y - (k_7 + k_8) XpY\\
%Y_p' & =  -k_{12} X_t Y_p - k_9 X_d Y_p + k_{10} XdYp + k_{13} XtYp + k_8 XpY\\
%XdYp' & =  k_9 X_d Y_p - (k_{10} + k_{11}) XdYp\\
%XtYp' & =  k_{12} X_t Y_p - (k_{13} + k_{14}) XtYp
%\end{aligned}
%\right.
\frac{d}{dt}
\left(
\begin{array}{c}
X_d\\
X\\
X_t\\
X_p\\
Y\\
XpY\\
Y_p\\
XdYp\\
XtYp
\end{array}
\right)
=
\left(
\begin{array}{cc}
-k_9 X_d Y_p - k_1 X_d + k_2 X + (k_{10} + k_{11}) XdYp \\
 k_1 X_d - (k_2 + k_3) X + k_4 X_t + k_8 XpY\\
 k_3 X - (k_4 + k_5) X_t - k_12 X_t Y_p + (k_{13} + k_{14}) XtYp \\
-k_6 X_p Y + k_5 X_t + k_7 XpY \\
-k_6 X_p Y + k_{11} XdYp + k_{14} XtYp + k_7 XpY\\
 k_6 X_p Y - (k_7 + k_8) XpY\\
-k_{12} X_t Y_p - k_9 X_d Y_p + k_{10} XdYp + k_{13} XtYp + k_8 XpY\\
 k_9 X_d Y_p - (k_{10} + k_{11}) XdYp\\
 k_{12} X_t Y_p - (k_{13} + k_{14}) XtYp
\end{array}
\right)
\end{equation}


%{\bf The structure of the file EnvZJ.nb}.
\BEN \im {\bf The   conservation laws}   are $X_d + X + X_t + X_p + XpY + XdYp + XtYp = x_{tot}$ (total EnvZ) and $Y + XpY + Y_p + XdYp + XtYp = y_{tot}$ (total OmpR).

 \im  the non-negative fixed points. \Ma's command Reduce takes lots of time here, but Solve[RHS==0,var] (the imperfect, quicker version) finds immediately three steady states. One is  the following RAP in terms of $X_t,X_p$:
\be{RAPJ} \bc X_d= \frac{k_2 \left(k_4+k_5\right)}{k_1 k_3}  X_t,X= \frac{\left(k_4+k_5\right) }{k_3}X_t,\\Y= \frac{k_5 \left(k_7+k_8\right)}{k_6 k_8 } \fr{ X_t}{ X_p},\text{XpY}= \frac{k_5 }{k_8} X_t,\\
Y_p= \frac{k_1 \left(k_{10}+k_{11}\right) \left(k_{13}+k_{14}\right) k_3 k_5}{k_1 k_3 \left(k_{10}+k_{11}\right) k_{12} k_{14}+k_2 \left(k_4+k_5\right) k_9 k_{11} \left(k_{13}+k_{14}\right)},\\
\text{XdYp}= \frac{\left(k_{13}+k_{14}\right) k_2 k_5 \left(k_4+k_5\right) k_9 }{k_1 k_3 \left(k_{10}+k_{11}\right) k_{12} k_{14}+k_2 \left(k_4+k_5\right) k_9 k_{11} \left(k_{13}+k_{14}\right)} X_t,\\
\text{XtYp}= \frac{k_1 \left(k_{10}+k_{11}\right) k_{12} k_3 k_5 }{k_1 k_3 \left(k_{10}+k_{11}\right) k_{12} k_{14}+k_2 \left(k_4+k_5\right) k_9 k_{11} \left(k_{13}+k_{14}\right)} X_t\ec,
\ee
which identifies again $Y_p$ as the ACR species.%

 There are also two
 boundary \fp s,  with six common invading components $X_d= X =X_ t=XpY =XdYp = XtYp = 0$. Under this condition, the steady points must still have $ X_p Y =0$. The first possibility
 is incompatible with the positivity
of the conservations, and the second,  $ Y= 0$, yields the DFE/invasion species set
\begin{gather*}
\{ X_d = 0, X = 0, X_t = 0, X_p = x_{tot},\\ Y = 0, XpY = 0, Y_p = y_{tot}, XdYp = 0, XtYp =0 \}
\end{gather*}
and resident species set $\{ X_p, Y_p\}$.


\im The next  step is to resolve the stability of the DFE by the ``all positive interactions NGM approach''. Here, the ``invading NGM matrix'' is of dimension 7, with 4 zero \eig s.
The stability reduces thus to the problem of ensuring that all the three roots of a cubic factor $ch(r)=0$ have real parts less than one.  Shifting the origin by $p(x)=ch(x+1)=x^3 + c_3 x^2 + c_2 x + c_1$ reduces this to the RH problem
$$c_1 \geq 0, c_2\geq 0, c_2 c_3 - c_1\geq 0,$$  which interestingly, depends on the species $Y_p$ only. Here
\BEN \im
The free coefficient is nonnegative precisely when \be{frc} y_{tot} \leq y_p^*=\frac{k_1 \left(k_{10}+k_{11}\right) \left(k_{13}+k_{14}\right) k_3 k_5}{k_1 k_3 \left(k_{10}+k_{11}\right) k_{12} k_{14}+k_2 \left(k_4+k_5\right) k_9 k_{11} \left(k_{13}+k_{14}\right)}\ee
\im The second coefficient is nonnegative when $y_l \leq Y_p \leq y_u$, where
$y_l, y_u$  are quite complicated, and involve square roots.
\im $ H_3=c_2 c_3 - c_1\geq 0$ is of order $4$ in $Y_p$, so solving \wrt\ this variable is impossible.
However, $H_3$ is linear in certain other variables, for example in $k_{13}$, which is hence removable. Now  the  simplified second coefficient, rather complicated, \mbw\
$\fr{n2}{(k_{10}+k_{11})d2}$, where
\begin{gather*} n2=-\left(\left(k_{10}+k_{11}\right) k_3 k_1^2 \left(k_8 k_{12} Y_p+k_5 \left(k_7+2 k_8\right)\right)\right)\\ +k_2 k_8 k_9 k_1 Y_p
\left(k_{11} k_{12} Y_p-\left(k_{10}+k_{11}\right) \left(k_4+k_5\right)\right)+k_2 \left(k_4+k_5\right) k_8 k_9^2 \left(-k_{11}\right) Y_p^2\end{gather*}
\begin{gather*}
  d2=k_3 k_1^2 \left(k_8 k_{12} Y_p+k_5 \left(k_7+2 k_8\right)\right)+\\ k_9 k_1 Y_p \left(-k_{12} k_2 k_7 Y_p +2 k_3 \left(k_8 k_{12}
  Y_p+k_5 k_7+2 k_5 k_8\right)+k_2 \left(k_4+k_5\right) k_8\right) + \\ k_9^2 Y_p^2 \left(\left(k_2+k_3\right) k_8 k_{12} Y_p+ \left(k_3 k_5+k_2 \left(k_4+k_5\right)\right)
\left(k_7+2 k_8\right)\right).\end{gather*}

Finally, the simplified positivity condition for the second coefficient along the manifold $H_3=0$, very
complicated, illustrates the fact that the stability domain $R_0$ of the DFE may be arbitrarily complicated when expressed in terms of the model parameters.
\iffalse
 Indeed, the all positive interactions NGM method reveals other conditions like
\be{mc} \bc (\sqrt{13}-3) k_1-2 k_9 Y_p>0\\
 k_5<\frac{k_1 k_{12} Y_p}{k_9 Y_p+k_1}\\
 k_4<\frac{k_1 k_{12} Y_p+k_1 k_5-k_9 k_5 Y_p}{k_9 Y_p+k_1}\\
 \ec
 \ee
 (among others) which might affect the stability of the DFE.
 \fi
\EEN
\EEN


 %\im We complete now the RH stability analysis of our third order polynomial,
%which requires executing Reduce[Append[cp,c1>0\&\&h3>0],Yp]




 We offer next, as an alternative to the ``maximal rank $F$'' method, which leads to a stability domain with a complicated boundary, a ``rank one F'' method. This approach yielded the same result in the example of Section \ref{s:EnvZs},  but here it  yields only the condition for positivity of the first coefficient of the \ch\ from the maximal rank $F$.  We conjecture therefore  that the rank one shortcut adopted below yields only part of the boundary of the stability domain (see also Open question 1).
\beR \lab{r:sh}
By only considering reaction $12$, which produces the ``infected'' species $XtYp$, as ``new infection'', we  decompose the gradient as
\begin{eqnarray*}
Gr =& \left(
\begin{array}{ccccccc}
 -k_9 Y_p-k_1 & k_2 & 0 & 0 & 0 & k_{10}+k_{11} & 0 \\
 k_1 & -k_2-k_3 & k_4 & 0 & k_8 & 0 & 0 \\
 0 & k_3 & -k_{12} Y_p-k_4-k_5 & 0 & 0 & 0 & k_{13}+k_{14} \\
 0 & 0 & 0 & -k_6 X_p & k_7 & k_{11} & k_{14} \\
 0 & 0 & 0 & k_6 X_p & -k_7-k_8 & 0 & 0 \\
 k_9 Y_p & 0 & 0 & 0 & 0 & -k_{10}-k_{11} & 0 \\
 0 & 0 & k_{12} Y_p & 0 & 0 & 0 & -k_{13}-k_{14} \\
\end{array}
\right) \no \\ =&F - V= \left( \begin{array}{ccccccc} 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & 0 & 0 & 0 & 0 & 0\\
 0 & 0 & k_{12} Y_p & 0 & 0 & 0 & 0 \end{array} \right) \no \\ & \; \; \; \; \; - \left( \begin{array}{ccccccc} k_9 Y_p+k_1 & -k_2 & 0 & 0 & 0 & -k_{10}-k_{11} & 0\\
-k_1 & k_2+k_3 & -k_4 & 0 & -k_8 & 0 & 0\\
0 & -k_3 & k_{12} Y_p+k_4+k_5 & 0 & 0 & 0 & -k_{13}-k_{14}\\
0 & 0 & 0 & k_6 X_p & -k_7 & -k_{11} & -k_{14}\\
0 & 0 & 0 & -k_6 X_p & k_7+k_8 & 0 & 0\\
-k_9 Y_p & 0 & 0 & 0 & 0 & k_{10}+k_{11} & 0\\
0 & 0 & 0 & 0 & 0 & 0 & k_{13}+k_{14}\end{array} \right)
\end{eqnarray*}
 The NGM matrix $K=FV^{-1}$ only has one nonzero eigenvalue which yields the basic reproduction number:
 {\footnotesize
\[R_0 = \frac{k_{12} ((-k_2 k_9 (k_{13} + k_{14}) y_{tot} + k_1 k_3 (k_{13} + 2 k_{14})) k_{11} + k_1 k_3 k_{10} (k_{13} + 2 k_{14})) y_{tot}}{((-y_{tot}^2 k_2 k_9 k_{12} + (k_1 k_{12} k_3 - k_9 (k_4 + k_5) k_2) y_{tot} + k_1 k_3 k_5) k_{11} + k_1 k_3 k_{10} (y_{tot} k_{12} + k_5)) (k_{13} + k_{14})},\]
}
and solving  $R_0 > 1$ for $y_{tot}$ gives
\[y_{tot} >y_p*, \]
the complimentary of \eqr{frc}, which is precisely the condition under which the positive ACR steady state exists. It follows that the boundary steady state loses stability the conservation law $y_{tot}$ crosses through the ACR value of $Y_p$.

This example shows that not all rank-one shortcuts provide the correct stability
conditions for the DFE (or at least, the answer they provide does not confirm that provided by the ``all positive interactions NGM method'').
However, since the full  Routh-Hurwitz analysis for stability is often  time consuming, or impossible,
the ``rank one  NGM shortcut'' seems worthwhile, even if it yields only part of the boundary of the DFE stability domain.\eeR



%\begin{equation}\label{eq:cons_envz2}
%\Cons=\spann \left\{
%\begin{pmatrix}
% 1 \\ 1 \\ 1\\ 1\\ 0 \\ 1 \\ 0\\ 1\\ 1
%\end{pmatrix},
%\begin{pmatrix}
% 0 \\ 0 \\ 0\\ 0\\ 1 \\ 1\\ 1\\ 1 \\1
%\end{pmatrix}
%\right\}
%\end{equation}
%}


\beO It has been observed in \cite{AABJ} and before  that sometimes selecting only
a subset of the infection/invading species leaves $R_0$ unchanged, while reducing the computations. Understanding when an ``$R_0$ sufficient minimal infection set'', different form the total infection set, exists, is an open problem, which might be related to the concept of siphons of the associated Petri net \cite{AdLSpetri}. \eeO



==> Lap.tex <==
\ssec{The representation as the product of the complex-composition, Laplacian and monomial rates}
We provide now one more representation used in CRNT, which applies only in the case of mass action kinetics (MAK) (or, slightly modified, for generalized
mass action  kinetics (GMAK)).

\be{Lr}x'= \Gamma \bf R(x)=(Y I_a) (I_k x^{Y})=Y \mL  x^{Y}.\ee Here  $Y$ is a $n_S\times n_C$ matrix whose columns specify the composition of the ``complexes" (i.e. the vectors representing the
left and right hand side of each equation), $I_a$ is the $n_C\times n_R$ incidence matrix of the \HJF\  graph on the complexes, whose edges correspond to the reactions, $x^{Y}$ is the  $n_C\times 1$ vector of exponents  of the inputs of each reaction, completed by $1$ for the complexes which are not inputs,
    and  $I_k$ is an $n_R\times n_C$ ``outgoing coincidence matrix" containing all the reaction constants, whose $(r, c)$-th element equals $k_r$ if the $c$-th complex is the input complex for the j-th reaction, and zero
otherwise.

It follows that $\mL=I_a I_k$ is a $n_C\times n_C$ ``Laplacian matrix" with non-positive diagonal elements and nonnegative off-diagonal
elements, whose all column sums  are  zero. This matrix intervenes in the study of ``complex-balanced equilibria" and Wegscheider conditions--see  for example \cite{Gater,van2015complex} for further details.





\beR \lab{r:reac}
Let us draw attention now to three advantages of decomposing RHS as in \eqr{SIRS}: \BEN
\im  The representation \eqr{SIRS} suggests that the investigation of CRN ODE's may be  split in two parts: ``structural elements" depending only on $\G$, and on the variables of each component of $ \bf R(x)$, and ``parametric elements" reflected in the specific structure of $ \bf R(x)$ (polynomial, or Michaelis-Menten, or Hill  kinetics, etc).
This opened up the fruitful investigation of ``robust questions" which are independent of the specific kinetics, like for example  ``robust stability", the  question of whether  the Jacobian of the RHS is a stable matrix independently of parametric kinetics.
\im  The problem of describing the fixed points becomes essentially trivial
when passing to ``reaction coordinates" defined by $ \bf R(x) = \bf z=(z_1, z_2,  ...)$. Indeed, on one hand, $\bf z$ must  belong to the null-space of $\Gamma$, and on the other hand $\bf z$ must be nonnegative, which means simply that
it is a non-negative combination of the extreme rays of the cone obtained by intersecting the  null-space with the non-negative cone. Now finding this cone is very easy for a computer algebra system (CAS): it simply requires adding the non-negativity constraint when solving $\Gamma \bf z=0$ for $\bf z$. At least, this problem is very easy when $\Gamma$ is numeric, which can always be ensured.
\im  When the \sm\ contains only $1,-1,0$ it represents the incidence matrix of an associated directed bipartite Petri/Volpert graph connecting the set of species with that of reactions. The intuitive graph representation helps, and ended up in inspiring  some of the robust Lyapunov function algorithms  in LEARN, which search for functions of the form $V(\bf R(x))$.

\EEN
\eeR



==> ME.tex <==
\section{Introduction to ME and CRN}

\ssec{Motivation}
 Chemical reaction networks
  (CRN)  (also called biological interaction networks (BIN) by some authors) and mathematical epidemiology (ME) have shared for long  common preoccupations, like the multi-stationarity and stability problems  (including that of boundary points, which lead to  the famous
$R_0 <1$ theorem in ME), and the bifurcations problem. \Fr  all these fields study  essentially non-negative ODE's, and their first historical tool has been checking  the {\bf Routh–Hurwitz-Li\'enard–Chipart criteria}, which unfortunately succeed symbolically only with few variables and parameters.

 Trying to develop more efficient methods for
 specific classes of larger ODE's, based on their  structure,   has been a  long-standing challenging goal in systems biology research. CRN/BIN researchers have developed remarkable tools, which include the Horn-Jackson-Feinberg and Petri/Volpert/DSR graphs, the ``deficiency'', the  ``conservations'' and ``positive fluxes'' of the {\bf \sm}, the  {\bf robust Lyapunov functions} (RLF), etc. (robust means here  that the determination of the fixed point(s) is not necessary  for defining the Lyapunov functions, since these are expressed in terms of
 the ``{\bf reaction variables}'', i.e. the nonlinear functions appearing in the RHS of the ODE, whose nullity defines the fixed points).

 {\bf Are there CRN and ME methods which might be useful in the ``sister science''?}
 The answer to this natural  question was  not at all obvious, since some important features in CRN examples, like zero deficiency (ZD) may probably never occur in ME (this is a consequence of the global attractor conjecture), and others, like weak-reversibilty, seem also impossible (this is an open question, whose answer depends on how we define ME models; our proposed definition is stated in Open Problem \eqr{o:MEm}). The   first positive answers to the question in the title of this paragraph were given in the
 recent paper Vassena \& al \cite{AAV}: \BEN \im One remarkable recent  result of \cite{Vas,VasStad}, which states that {\bf any auto-catalytic CRN will admit  unstable equilibria (increasing thus the chance of Hopf bifurcations), if all the reaction rates are ``rich enough''}, for example \MM\ (MM), lead in ME to  \cite[Thm 3.1]{AAV}.  The latter  may be stated as:
      ``Consider any epidemiological system in which there exists an ``$S\to I$ infection  reaction'' with ``admissible rate'' $R_1(s,i)$, and an ``$I\to ...$ treatment  reaction'' with  ``admissible rate'' $R_2(i)$, where admissible is defined in the original papers, and also here below, in Remark \ref{r:adm}. Then, the ``symbolic Jacobian'', in which $R_1,R_2$ are not specified (but the sign of their derivatives
      is specified, via admissibility), may always have purely imaginary eigenvalues if $R_1,R_2$ are ``rich'' in the sense of \cite{Vas,VasStad} (for example, \MM).

      Briefly,
 all  epidemic models admit ``symbolic  bifurcations'', provided their rate functions  have enough parameters;  it is only the restriction
to mass action that may prevent the occurrence of Hopf bifurcations.

Note that this result had been observed  empirically in many particular three compartment SIR-type models, but the fact that the  number of  compartments and the exact architecture of the model are irrelevant, was not understood.

     Note also that since in ME it does  not make  much sense to replace  linear rates by \MM,  the result  in \cite{AAV}, which only assumes the ``relevant'' rates to be rich,
        required a careful  reexamination of the method of \cite{Vas,VasStad}.
       % A related example is provided here in section \ref{s:SIRScap}.
       \im A second CRN result  exploited in \cite{AAV} was the {\bf Inheritance of oscillation in chemical reaction networks} of  \cite{banaji2018inheritance}, which gives conditions for Hopf  bifurcations to be inherited by models, given that they exist in a sub-model where some parameters are $0$.
  This allowed establishing the existence of  Hopf  bifurcations for the mass-action ME model %\eqr{SIRn} below
  (using their existence in the case of no demography, already established by Hethcote and Van den Driesche \cite{HethSVDD}).
  \im In the opposite direction, we show below that the \NGM\ method of
  \cite{Diek,Van,Van08}, may be applied to find conditions for  the stability
  of fixed boundary points of interesting CRN models.
\EEN



\subsection{How to parameterize ME and CRN models?}

 For the second  question  formulated in the title of this section,
  how to parameterize  ME  models,
   there are three natural choices.


 \BEN \im
 The parametrization   used traditionally for ODE models in ME  is as a pair (RHS, var), where RHS denotes the set of formulas for the derivatives, and var are the  variables whose rates of change we study.
 This parametrization is well geared for solving symbolic bifurcation problems for small size models. It ignores though the ``network" (or graph) structure revealed by the following two parametrizations.


  \im Chemical reactions networks research  suggests that a model should be defined by a triple $(\G, {\bf R}, x)$, associated to the decomposition \be{crnsys}x'=RHS=\G .{\bf R}(x)\ee
  \BEN \im where $x$ denotes the variables \im
   $\G$ is the ``stoichiometric matrix'' (SM), whose columns  represent directions in which several species/\com s change simultaneously,
   \im  ${\bf R}(x)$ is the  vector of rates of change associated to each direction, also known as kinetics.
    \EEN

For example, here is the  triple $(\G, {\bf R}, x)$ of the  simplest
 SIRS ODE:
  \be{SIRS0}
x'=\bep
\s' \\\iem  ' \\\r' \eep =  \bep - 1&0&1&-1 \\
  1&- 1&0&0\\
  0&1&- 1&1
\eep \bep
\b \s  \iem   \\ \g_i \iem   \\ \g_r \r \\ \g_s \s  \eep:=\Gamma {\bf R}(x)
\ee
(with $\l=\mu=\de=0$ as compared to \eqr{SIRS} below,  for ease of display).

The rates $R(x)$ must satisfy admissibility conditions -- see Definition \ref{d:R} below.

This parametrization is geared for studying ``robust questions" like for example the existence of ``robust Lyapunov functions " which depend only on the ``reaction variables $\bf z={\bf R}(x)$~\cite{Franco,al2014robust}.


%%%%%%%%%%%%%%%%%%%%%
   \im Yet a third parametrization used in CRN is to enter for each column of $\G$/``reaction" its traditional ``mass-action'' CRN representation   as a pair ``(input $\to$ output)'', in the style
    $$I\to R, ...$$ (this reaction represents in SIR recovery  after being infected),
    each reaction being  a directed pair consisting of the ``source complex'',  and a ``product complex'' see  definition below.

    \beD \lab{d:CRN} A {\bf mass-action} CRN is defined by a triple $\{\mathcal{S},\mathcal{C},\mathcal{R}\}$, where $\mathcal{S},\mathcal{C},\mathcal{R}$ are the set of species, complexes and reactions respectively.

\begin{align*}
    \mathcal{S} &= \{S_1, ... , S_i,..., S_{|\mathcal{S}|}\}\\
    \mathcal{C} & = \{y_1,...,y_\alpha,...,y_{|\mathcal{C}|} :y_\alpha \in \mathbb{N}^{|\mathcal{S}|}\}\\
    \mathcal{R} &= \{ \ce{ y_{\alpha} ->[k_{y_{\alpha} \to y_{\beta}} * x^{y_{\alpha}}] y_{\beta} } : k_{y_{\alpha} \to y_{\beta}} \geq 0\},
\end{align*}
where Roman letters ($i,j$) and Greek letters ($\alpha,\beta$) are used to denote species and complex indices, respectively, and $x=\{s_1, ... , s_i,..., s_{|\mathcal{S}|}\} $ denotes the vector of unknowns.
A complex is a multi-set of species, and is denoted by the column vector $y_\alpha$ representing the stoichiometry/direction of the multi-set.
\eeD

  \beXa {  The SIRS ODE \eqr{SIRS0} is induced by the reactions:}
{
\be{RNSIR} \bc  \ce{ S + I ->[\beta s i] 2I}\\ \ce{ I ->[\gamma_i   i] R } \\
 \ce{R ->[\g_{r} r] S } \\
 \ce{  S  ->[\g_{s} s] R } \ec \ee
}

From this representation,  one may construct the stoichiometric/directions matrix $\Gamma$, by associating to each reaction   a column   given by $ y_{\beta}-y_{\alpha}$,  and also recover  the  derivatives of the variables collected in RHS, in the first representation.

In this example, \begin{align*}
    \mathcal{S} &= \{S,I,R\}, x=(s,i,r),\\
    \mathcal{C} & = \{y_1=(1,1,0),y_2=(0,2,0),y_3=(1,0,0),y_4=(0,1,0),y_5=(0,0,1) \}\\
    \mathcal{R} &= \{ \ce{ y_1 ->[\b  x^{y_1}=\b s i] y_2}, \ce{ y_4 ->[\g_i  i] y_5},...\},
\end{align*}\eeXa




\EEN

\beR The last three reactions of \eqr{RNSIR} are self-explanatory, but not the first; this one is a consequence of adopting the mass-action representation of our ODE, which requires that the linear coefficients multiplying $S,I$ on the LHS of  \eqr{RNSIR} equal the exponents of $s,i$ in the rate of the reaction.
\eeR



\beR   A variant of the last representation is to provide a ``sources matrix", which gathers  the coefficients of all the LHS of the reactions,
and a ``products matrix", which gathers  the coefficients of all the RHS of the reactions, This is used typically in the Matlab and python packages
(for example, those listed in Section \ref{s:res}).

We prefer using  the Mathematica package Reaction Networks \cite{Toth},  which provides in one command, ``ReactionsData'', many important network characteristics like the  stoichiometric matrix,  the RHS (associated to  mass action),   the \FHJ\ (FHJ) graph on the complexes,  the  Petri/ Volpert/DSR complexes-reactions bipartite digraph, etc. %for a nice parallel display of several aspects of a single CRN ODE, see
  %for example \cite[Fig. 2]{AAScomp}.

\iffalse has been used in the Harvard lab package reaction-networks.m, developed by Robert L. Karp and modified later by Tathagata Dasgupta and Joseph P. Dexter,
available at

\url{http://vcp.med.harvard.edu/software.html}

Here the input  is a list of reactions, with  a third element, r, being added to each pair, for reversible reactions. Unfortunately, this package utilizes common symbols with ReactionKinetics, like for example  ``Reactions'', and so the two require further changes before they can  be used together.
\fi

  \eeR

\subsection{What are ME  models?}

Note first that a definition of ME models is still lacking.
One might want to ask for essential non-negativity, but  for a counterexample see  \cite{Rodrigues}.  We might also want to rule out types of reactions absent in all
epidemiological models, like simultaneous degradations (deaths), written by chemists in the form ``A''+''B''$\to$0, and ``two from one reactions'', like ``C''$\to$''A''+''B''. It seems premature now   to  speculate on this question;
 however, as a wide digression, we conjecture  that
\beO \lab{o:MEm}
A definition of mass-action ME models should identify an appropriate  subclass of the class of
chemical reaction networks, possibly the subclass including only transfers (monomolecular reactions), and bimolecular reactions of the types $S+E\to 2 E, S+I\to I+E$, as encountered in SEIR.\eeO
%systems admitting a BDC-decomposition in the sense of \cite{GiuliaFranco}, which includes already all , and also flow and compartmental systems (for a survey see \cite{Giulia}).  We identify this as a direction for future work.




\ssec{The admissibility conditions for reaction rates}

\beD \lab{d:R}  A BIN/CRN is an ODE admitting a (non-unique) representation with rates satisfying the following
{\bf admissibility restrictions} \cite{ARS24}:
  \begin{enumerate}
    \item $R_i(x)$ is $C^1$ (continously differentiable).

    \item

      \begin{gather*}\frac{\partial R_i(x)}{\partial x_j}
    \begin{cases}
        \geq 0 & \text{if $x_j$ is a reactant} \\
        \leq 0 & \text{if $x_j$ is a product} \\
        = 0  &\text{otherwise}
    \end{cases}, \\
    \frac{\partial R_i(x)}{\partial x_j} \;
    \begin{cases}
        >0 & \text{if $x_j$ is a reactant and all the reactants are present} \\
        <0 & \text{if $x_j$ is a product and all the products are present}
    \end{cases}
  \end{gather*}

      \item
        \begin{gather*}R_i(x)
    \begin{cases}
        \geq 0 & \text{if not all products are present} \\
        \leq 0 & \parbox[t]{.6\textwidth} {if not all reactants are present (which rules out mass-action and \nc\ BINs, for example)}
      \end{cases}\end{gather*}

\end{enumerate}


\eeD



   \ssec{A bird's eye view of CRNT }
    CRNT might be divided in three  directions:
    \BEN \im The study of mass-action kinetics (MAK), like SIRS, with further examples  provided throughout the paper. These may further be divided in non-catalytic and
     {auto-catalytic}.
    \im The study of generalized mass-action kinetics (GMAK).
\im The ``robust'' study of {non-catalytic CRNs}, which generalizes mass-action kinetics by replacing the nonlinear interactions with arbitrary admissible functions -- see Remark \ref{r:adm}. One studies then
     ``robust stability and non-oscilation'' -- see  for example \cite{EfimovgLa,AAnew,AAScomp,AASrob,Ali23gr}. %and Definition \ref{d:RLF} below.

    While not directly applicable in ME,  which concerns auto-catalytic CRNs, mentioning this sub-field   is unavoidable in a paper on computational tools, (in the ArXiv version), due to their
    powerful algorithmic tools encapsulated in
LEARN. %, and to the hope that extensions applicable to ME might be possible.%. We provided several {\bf CRN examples} in section \ref{s:rob}, in

     \EEN





==> SIR1S.tex <==

%\newpage
\subsection{The mass-action SIR1S, where the recovered may also infect,  does not
admit \Hb: SIR1S.nb, SIR1S.jl (3,9,3,2)}\lab{s:SIR1S}
{

We discuss now   the particular case $n=1$ of the   SIRnS model \cite{Carlos,AAV}, with a \sm\ involving $9$ reactions:
\begin{gather}\label{SIR1S}  \nonumber\begin{pmatrix} s'\\i'\\r '\end{pmatrix}=\left(
\begin{array}{ccccccccc}
 1 & -1 & 0 & 0 & 1 & -1 & -1 & 0 & 0 \\
 0 & 1 & 1 & -1 & 0 & 0 & 0 & -1 & 0 \\
 0 & 0 & -1 & 1 & -1 & 1 & 0 & 0 & -1 \\
\end{array}
\right) \left(
\begin{array}{c}
 \lambda  \\
 \beta  i s \\
 i r \beta _r \\
 \gamma  i \\
 r \gamma _r \\
 s \gamma _s \\
 \mu  s \\
 i \mu  \\
 \mu  r \\
\end{array}
\right) \\ =
\left(
\begin{array}{c}
- \beta   s i+\lambda +r \gamma _r-s \gamma _s-\mu  s \\
 i \left(-\gamma -\mu +r \beta _r+\beta  s\right) \\
 i \left(\gamma -r \beta _r\right)-r \left(\mu +\gamma _r\right)+s \gamma _s \\
\end{array}
\right)\end{gather}
It has one  parameter $\beta _r >0$, the rate at which the (partly) recovered can still infect, which was not present in SIRS, and we have also added another often used parameter $\gamma _s$, which seems not to affect  the essence of the results, but does affect execution times.


The normal situation is $\beta _r < \beta $, but the opposite may happen for ``perverse viruses".

The deficiency  is $2$, more than for SIRS. %We will however propose a

\beR We can also represent the model via its reactions
RN=\{$0\to "S","S"+"I"\to 2 "I","I"+"R"\to  2 "I","I"\to "R","R"\to "S","S"\to "R","S"\to 0,"I"\to 0,"R"\to 0$\}.

Notice that, leaving aside  the usual input  and output reactions, we have only two types of reactions: infections like "S"+"I"$\to$ 2 "I", and transfers like "I"$\to$ "R".  The maximum possible number of reactions after this restriction is $2+6=8$. Note that in CRN, \cite[Lem 3.4]{BanBor} have found 6486  non-equivalent, non-equivalent bimolecular (3,4,3) models, and proved the presence of non-degenerate Hopf bifurcations  in  86 of them
\cite[Thm 5.2]{BanBor}.

The SIR1S without demography is a (3,5,3) model, and we show below that
it does not have \Hb.

An open question, in the style of \cite{BanBor}, is:
\beO Does the extended SIR1S of type (3,8,3), where we have added all the possible linear transfers (which may all be interpreted epidemiologically, and have in fact appeared individually in the literature), admit \Hb? \eeO

A more ambitious open question is:
\beO Identify which SEIR-type models  admit \Hb, where we define
SEIR-type to mean CRN bimolecular models with 4 species and maximal rank, and only reactions of transfer and  of infections of the types $S+E\to 2 E, S+I\to I+E$.  \eeO
\eeR

The DFE of SIR1S is the same as for SIRS, but $R_0$ is more complicated, due to the new ``infection path" via the recovered.
$$ R_0= \sd \frac{\beta  }{\gamma +\mu }+\rd\frac{ \beta _r }{\gamma +\mu }$$
Note both the DFE and $R_0$ simplify considerably when $\g _s=0$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\sssec{Rational univariate representation (RUR)  for SIR1S}
Via Groebner  elimination implemented in our RUR script, we find that
(as often is the case) $s,r$ have rational expressions in terms of $i$,  with positive coefficients. The respective formulas are:

\be{csr}s= \frac{i \mu  \beta _r+(\gamma +\mu ) \left(\mu +\gamma _r\right)}{\beta  i \beta _r+\beta  \left(\mu +\gamma _r\right)+\beta _r \gamma _s},
r= \frac{\beta  \gamma  i+(\gamma +\mu ) \gamma _s}{\beta  i \beta _r+\beta  \left(\mu +\gamma _r\right)+\beta _r \gamma _s}.\ee



 These substitutions allow  replacing the fixed point system
by an equivalent rational univariate representation (RUR) scalar polynomial equation in $i$. After dividing by $i$, the endemic point satisfies a quadratic equation:
\be{polSIR1S} 0=P(i)= a_2 i^2+a_1 i+a_0 ,\ee where
\be{co1} \bc a_2 =\mu  \beta  \beta _r  %\left(\gamma/\mu +1\right)
>0
\\a_1 =\beta  \mu  \left(\gamma +\gamma _r\right)-\beta  \lambda  \beta _r+\mu ^2 \left(\beta +\beta _r\right)+\mu  \beta _r \gamma _s\\
a_0= \left(\mu +\gamma _r\right) (\mu  (\gamma +\mu )-\beta  \lambda )+\gamma _s \left(\mu  (\gamma +\mu )-\lambda  \beta _r\right)=\mu(\gamma+\mu) \\
(\gamma_r+\gamma_s+\mu)(1-R_0).\ec\ee
%a_0=\left(\mu +\gamma _r\right) \left(\mu  \left(\gamma +\mu _i\right)-\beta  \lambda \right)=\mu  \left(\gamma +\mu _i\right)\left(\mu +\gamma _r\right) \left(1-R_0 \right).

Analyzing the sign of the coefficients, we find
that there may be  two endemic points.  More precisely
{
\BEN \im If $  R_0 >1,
$   there is  precisely one positive endemic point, which turns  out to be always stable.
\im  If $R_0 < 1 \Eq  a_0 >0$, unlike SIRS, there may be two positive endemic points, provided $\b \geq \b_D$ (where $\b_D$ is the largest root of the discriminant),  $\b \leq \b_r$ , and the following further   conditions hold:
 \be{2pr}\bc { \lambda \beta _r \gamma}  > \mu(\gamma +\mu )(\gamma +\mu +\gamma _r)\\ \gamma _s<\gamma _{s,M}:=\frac{\mu  \left(\mu +\gamma _r\right)
[\mu (\mu +\gamma)(\mu +\g+ \gamma _r)  -\gamma  \lambda  \beta _r]}{\mu ^4+\mu ^2 \left(\gamma  \left(\gamma +\gamma _r\right)-\lambda  \beta _r\right)-2 \gamma  \lambda  \mu  \beta _r+\lambda ^2 \beta _r^2+\mu ^3 \left(2 \gamma +\gamma _r\right)}\ec\ee
The conditions above were obtained in 130 secs by

 \begin{lstlisting}[language=Mathematica]
Reduce[Append[cp,dis>=0\&\&a0>0\&\&a1<0\&\&$\beta$<$\beta$ r],$\beta$]//FullSimplify
\end{lstlisting}
where cp are the positivity conditions, and $dis$ is the discriminant of $P(i)$.
It may be checked that under the first condition in \eqr{2pr}, which restricts $\mu$ to be small,  the denominator of $\gamma _{s,M}$  is always negative, and hence $\gamma _{s,M}$
is positive.


\EEN
\beR   The  discriminant of the polynomial \eqr{polSIR1S} (provided in the \Ma\ file), is a second order polynomial in all the variables except $\mu$ (which appears with exponent 4), and hence no parameter  may be rationally explicitized.
\iffalse
Explicitizing \wrt\ $\b$ (our favorite bifurcation parameter) yields:
$$\b=\frac{\beta _r  \mu ^2}{\beta _r  \Lambda  +\mu  (\gamma +\mu )+\gamma _r (2 \gamma +\mu ) \pm 2 \sqrt{ \gamma   \left(\gamma _r+\mu \right) \left(\beta _r  \Lambda  +\gamma _r (\gamma +\mu )\right)}}(<\beta _r ).$$

\fi

%3) The  discriminant of dis \wrt\ $\l$ is  $\beta ^3 \left(\beta _r -\beta \right) \beta _r ^2 \gamma  \mu ^2 \left(\gamma _r+\mu \right)$. We confirm thus the result of \cite{AAV} that  there is no SN bifurcation when $n=1, \beta _r <\beta$.
\eeR

\sssec{A rational ``mixed var-par" parametrization for SIR1S}



Since further eliminating $i$ gives rise to lengthy computations, we have explored in the Mathematica file  an alternative: a rational parametrization  obtained by completing   \eqr{csr} with a solution of $P(i)=0$ with respect to some parameter
%$$\lambda \to \frac{\mu  \left(\beta  i^2 \beta _r+\beta  i \left(\gamma +\mu +\gamma _r\right)+i \mu  \beta _r+(\gamma +\mu ) \left(\mu +\gamma _r\right)\right)}{\beta  \left(i \beta _r+\mu +\gamma _r\right)}$$
 $$\lambda\to \frac{\mu  \left(\beta  i^2 \beta _r+\beta  i \left(\gamma +\mu +\gamma _r\right)+i \beta _r \left(\mu +\gamma _s\right)+(\gamma +\mu )
\left(\mu +\gamma _r+\gamma _s\right)\right)}{\beta  i \beta _r+\beta  \left(\mu +\gamma _r\right)+\beta _r \gamma _s.}    $$
(this includes $i$).

Under this parametrization, it is possible to solve $H3=0$ (where $H3$ is defined in \eqr{H3}), yielding also $\g$ as a rational  function, displayed only in the case $\g_s=0$, to
improve readability,
%$$\frac{(\beta  i+\mu ) \left(i \beta _r+\mu +\gamma _r\right) \left(\beta  i \mu _i+\left(i \beta _r+\mu +\gamma _r\right) \left(i \left(\beta +\beta _r\right)+2 \mu +\gamma _r\right)\right)}{i \left(\beta -\beta _r\right) \left(\mu +\gamma _r\right) \left(i \left(\beta +\beta _r\right)+\mu +\gamma _r\right)}$$
$$\g=\frac{((i \beta+\mu) (i \beta_r+\gamma_r+\mu) (i \beta_r+\gamma_r+2 \mu))}{(i (\beta_r-\beta) (\gamma_r+\mu))},$$
which is always positive when $\beta _r>\beta$.


 Finally, under this further substitution, the first two coefficients
of the \ch\ turn out to be $\left\{- \mu ^2 \left(i \left(\beta +\beta _r\right)+2 \mu +\gamma _r+\gamma _s\right),-\mu ^2\right\}$, hence always negative, while the third is positive.

At this point, we know that for $R_0>1$,  \Hb\ is impossible for the unique \enp. It is then natural to ask:
\beO For $R_0>1$, is the  unique \enp\ of SIR1S globally asymptotically stable?\eeO



==> SIR2S.tex <==
\subsection{SIR2S without vaccination admits Hopf and \dzb: SIR2S.nb (4,11,4,3)}\lab{s:SIR2S}
This process is similar, but harder than SIR1S (for example it's \defi\ is $3$), and it becomes crucial to perform the Mathematica computations in a convenient order, to avoid kernel crashes because of excessive execution time.

\BEN \im The first cell finds there are four fixed points, identifies the DFE, and shows that the \ch\ of the Jacobian at the DFE has 4 linear factors, but only one eigenvalue which may be positive. Next, we  obtain a   \rap\ of the interior fixed points, (similar to that for SIR1S), by solving $s,r_1,r_2$ \wrt\  $i$ and    completing the set of variables $s,r_1,r_2$ by one parameter which may be solved linearly from the RHS, in this case $\l$. Finally, we replace $\l$ in the list of parameters by $i$ (which satisfies a  third degree polynomial). This way, we have  circumvented the  multi-stationarity problem.
Under the new parametrization of the fixed points,   everything is explicit, including the coefficients
of the \ch\ of \jac\ at an \enp, under \rap. We also test the unconditional positivity of the coefficients, i.e. whether they
are sums of positive terms only. Here, we find that they may change sign. Since they are exceedingly long, we use the ``OnlyP" function  defined in our Epid-CRN package, to d
etect the presence of  minuses in the (simplified) expressions.
\im

The second cell solves in 0.67sec the conditions  co1=0, co2=0 for double zero bifurcation on $\b,\g$
(which are the variables of smallest degree). There are two solutions.  Both of them are too long to be displayed in the paper, and from now on we start to focus on the case
$\g_2=0$, (in ME this would be called  SIR2), not for SIR2S.  It is found that  the positivity of one of the solutions is incompatible with the other positivity conditions on $i$,
and the parameters. This takes 45.09sec when $\g_2=0$, and more than three hours \oth.
From now on, only the case  $\g_2=0$ is pursued.

\im The third cell finds the conditions \eqr{bb} in the theorem below.

\im The fourth cell computes the Hurwicz determinant $H_4$, and discovers it has two factors, both of which have sign changes.

Both of these two factors turns out to be $0$   under the double zero condition,
and hence
candidate for \Hb, in 347.78sec, and 16.85min, \resp.
\im The fifth cell  attempts to find even simpler particular cases for which we have \dzb, but this turns out impossible.
\EEN

The above suggests the following:
\beO
 \BEN \im For any $\g_1>0, \mu>0, i>0$ the model $SIR2$, with $\g_2=0,$ admits endemic equilibria with   Jacobian having a double zero,  where $\l, \b,\g$ are rational functions of the other parameters and $i$, provided
  certain  rational equalities and inequalities, necessary for the positivity of $\b,\g$ and provided only in SIR2S.nb, are satisfied.


For example, when $\g_2=0,$  the necessary inequalities  mentioned above, which ensure
the positivity of $\b,\g$, are
\be{bb}\beta _2<\beta _1<\beta _2 +\frac{\gamma _1 \mu +\beta _2 i \mu +\mu ^2}{\beta _2 i^2}.\ee

 \im On the double zero manifold of part 1., the Hurwitz determinant $H_4$ is doubly identically $0$, suggesting a degenerate Hopf bifurcation occurs.

 Establish the existence of Hopf and \BTb\  for SIR2S, and prove that the Hopf manifold $H_4=0$ has a double contact with the BT manifold $co_1=0=co_2$, for SIR2S, with $\g_2=0$.
\EEN
\eeO



\iffalse
$$\bc \l=\l_{BT}= \frac{(b_0+b_1) \mu  \left(b_1 \left(b_1 \left(\gamma _0+\mu \right)-b_0 \gamma _0\right)-b_0^2 \gamma _0\right)}{\left(b_1 \mu -b_0 \gamma _0\right) \left((b_0+2 b_1) \gamma _0+b_1 \mu \right)},\\\gamma _1=\frac{\left(\gamma _0+\mu \right) \left((b_1-b_0) b_1^2 \gamma _0 \mu +b_0^2 (b_0+2 b_1) \gamma _0^2+b_1^3 \mu ^2\right)}{(b_0+b_1)^3 \gamma _0^2}\ec\,$$
provided that
\eqr{neq1} hold and that $b_0> b_1$.


\prf For  $n=1$, the equations co1=0, co2=0 are easily solved \wrt\ $\l,\g_1.$ \QED
\beR Assuming $\l=\mu_i=\mu$ allows one, by restricting to initial conditions on the invariant manifold $s + i + \sum r_k=1$, to study the slightly simpler closed problem:
\bea && \bep s'\\i'\\r'\eep=
 \bep
-\b&0\\
\b&\beta _1\\
0&-\beta _1 \eep
\bep -\gamma _s &\mu&\mu+\gamma _r\\0&- \left(\gamma +\mu \right)&0\\
\gamma _s&\g&- \left(\mu +\gamma _r\right) \eep.
\bep  s i \\  r i \\ s\\i\\r\eep
\eea

But in this case the conservation equation must be added to the system.  We have chosen an intermediate solution. We assume only $\mu_i=\mu,$ which reduces sometimes execution times, but report on  the results  in the Mathematica file
only when also $\l=\mu,$  for simplicity.
\eeR
\fi




 \iffalse
 %Note that \cite{Earn24} analyzed
%recently the first passage properties we generalize here   of  by allowing for positive  $\g_r,\g_s$.
\beR
 \cite{Earn24}  connect the
deterministic/fluid limit models like \eqr{SIR1S} with the branching process approximation which is valid when $i$ is small. They start thus with   random walk processes $(S_n,I_n,R_n)$, which depend on the expected total population $n$, and approximate then the ``infectious projection" $I_n$  by a birth and death process  with birth rate
$\b X(t) +\beta _1 Z(t),$ where $X(t)=\fr{S_n}n, Z(t)=\fr{R_n}n$, and with death  rate $\mu +\g$.  Consequently, they apply a formula of Kendall \cite{Kendall} for the
extinction probability of a birth and death process with time-inhomogeneous rates, using different approximations for a ``fizzle" and for a ``burnout".

For a fizzle, one may use the slow system in the critical manifold $I=0$, which in our case is:
\bea \bep s'\\r'\eep=\bep -\left(\mu +\gamma _s\right) & \gamma _r\\\gamma _s&- \left(\mu +\gamma _r\right)\eep \bep s\\r\eep +\bep \mu\\0\eep,\eea
starting at the DFE, which implies that the extinction probability is $1/R_0$.
\eeR
\fi

\iffalse
We provide next conditions for the existence of Hopf, saddle-node and Bogdanov-Takens bifurcation points, obtained with Mathematica "helped by the programmer" (the problems are already too time-consuming otherwise).   Note that the solutions may be expressed in terms of the original parameters,  in terms of $\bff x$  only,  in terms of $\bff b$  only, in terms of $\bff x, \bff b$, or in terms of $\bff x,  b_1, \g_1$. We provide several alternatives, for comparison, and note that the direct approach of removing the dependence on $i$ via Groebner bases or resultants is quite cumbersome, resulting in an object which is a product of 26 factors!


\begin{theorem} Let SIR1S with $\gamma _s=0$ be defined by:
\bea
\bc
s'=-s (\beta  i+\mu )+\lambda +\gamma _1 r,\\
i'=-i \left(\gamma _0+\mu \right)+\beta _1 i r+\beta  i s,\\
r'=\gamma _0 i-\beta _1 i r-r \left(\gamma _1+\mu \right).
\ec
\eea

A) In terms of $\bff b$, the system $SIR1S$ admits positive endemic equilibria with a singular Jacobian
if $$\l=\l_c=\frac{(b_0+b_1) \mu  \left(\gamma _1 \left(b_1^2 \mu -b_0 (b_0+2 b_1) \gamma _0\right)-b_0^2 \gamma _0 \left(\gamma _0+\mu \right)\right)}{b_1 \left(\gamma _0+\mu \right) \left(\gamma _1+\mu \right) \left(b_1 \mu -b_0 \gamma _0\right)},$$
which is positive provided that
\be{neq1} \bc \mu {b_1}< \gamma _0 {b_0 }\text { or}\\ \gamma _1>\frac{b_0^2 \gamma _0 \left(\gamma _0+\mu \right)}{b_1^2 \mu -b_0 (b_0+2 b_1) \gamma _0}, \mu \frac{b_1^2}{b_0 (b_0+2 b_1) }> \gamma _0\ec.
\ee

B) In terms of $\bff x,  b_1, \g_1$, the system $SIR1S$ admits positive endemic equilibria with a singular Jacobian
iff ...

C)  In terms of the original parameters, the system $SIR1S$ admits positive endemic equilibria with a singular Jacobian
if ...


\end{theorem}
\prf For  $n=1$, the equation co1=0 is easily solved \wrt\ $\l$, and the positivity conditions for $\l_c$ are as stated above.
\QED







\beR To generalize for arbitrary $n$, we must show that for any matrix of the form $V^{-1}\T B$, where $\T B$ is stochastic, and  $V^{-1}$ has only positive elements, it is possible to choose a diagonal positive matrix $diag(\bff x)$ so that their difference is singular.

\eeR

\beXa  We provide now a bifurcation diagram in terms of $\g_1$, with  the  parameters $i,r, b[1]$ chosen arbitrarily, and $s$ chosen so that $\l$ takes its critical value. We obtain then expressions of the other parameters (except $\l$) in terms of the chosen values for $s,i,r, b[1]$ and $\g_1$.

%The resulting  RHS is

\eeXa

Before proceeding, let us discuss  the issues facing the programmer for the Hopf problem.  For  $n=1$, the  necessary conditions for a Hopf point
are $cHopf=\set{co2 co3-co1 co4=0,  co1\geq 0, co2\geq0, cp}$, where cp are the nonnegativity conditions of the parameters. \Ma\ cannot resolve this system, but can deal with the first condition only,
 and one of the  solutions obtained is provided above, \wrt\ $\l$ or $\g_1.$
 The programmer may prune solutions with negative parameters by inspection. Finally, he needs to ensure that the values obtained for $\l$ or  $\g_1$  are positive, and that the remaining ignored conditions $cRH=\set{ co1\geq 0, co2\geq0}$  are \satd.
\begin{theorem}
The Hurwitz determinant H3 of  $SIR1S$  is $0$ iff
if $$\bc \l=\l_{H}=\frac{(b_0+b_1) \mu  \left(b_0 \gamma _0-b_1 \mu \right) \left(\gamma _1^2 \left((b_0+2 b_1) \gamma _0+b_1 \mu \right)+\gamma _0 \gamma _1 \left(b_0 \gamma _0+3 b_0 \mu +2 b_1 \mu \right)+b_0 \gamma _0 \mu  \left(\gamma _0+\mu \right)\right)}{\left(\gamma _0+\mu \right) \left(\gamma _1+\mu \right) \left(\mu ^2 \left(b_1^2 \left(-\gamma _1\right)-2 \left(b_0^2+b_1 b_0+b_1^2\right) \gamma _0\right)+\gamma _0 \mu  \left(b_0 b_1 \gamma _0-\left(b_0^2+b_1 b_0+2 b_1^2\right) \gamma _1\right)+b_0 b_1 \gamma _0^2 \gamma _1+b_0 b_1 \mu ^3\right)}\\
\text{ or } \g_1=\g_{1H}=-\frac{\mu  \left(\gamma _0+\mu \right) \left(\gamma _0 (b_0 b_1-(b_0+b_1) \lambda )+b_0 b_1 \mu \right)}{(b_0+b_1) \gamma _0 \left((b_0+b_1) \mu -\lambda  \left(\gamma _0+\mu \right)\right)}\ec,$$

 In both cases, positive endemic equilibria with   pure imaginary eigenvalues
 may not be achieved with positive parameters?


%The system $SIR2S$  admits endemic equilibria with   pure imaginary eigenvalues and positive parameters if

\end{theorem}
\prf As mentioned, \Ma\ cannot handle all the  conditions for Hopf, but is able to factor H3 and obtain thus the two cases listed above. But the positivity conditions are impossible to achieve? \QED

\beR \lab{r:ngm}

Note that $B,V$ introduced above are related of the classic $\T F,\T V$  (new infections and interactions) of \ME, which intervene in the \NGM\ approach.  We recall this approach consists in denoting by $\T F,\T V$, the projections of $F,V$ on the coordinates which become $0$ at the DFE, and expressing
 the stability of the \DFE\  as $R_0<1,$ where $R_0$ is the spectral radius (and Perron-Frobenius eigenvalue) of the ``next generation matrix" $\T K=\T F (\T V)^{-1}$ evaluated at the DFE. Our approach shows that the full matrices $B,V$ are also relevant for the analysis of any fixed point. % to express the stability domain of any fixed point as $R_0<1$, where $R_0$ is the spectral radius of  $K=F V^{-1}$, evaluated at that point.  This turns out quite easy for models which have rational fixed points like SEIAR, SIRUV, multistrain, etc.

  Finally, we may also give   conditions for  bifurcation points in terms of the $\xi$ coefficients of the generalized eigenvalue problem
$ch(\xi):=\det\pp{  F -\xi V}$ \red{?}.

 \eeR
 \fi

 \beO The  multi-stationarity and multi-stability of SIRnS are
open problems, for $n > 2$.
\eeO


==> SIRSd.tex <==
%\newpage

\section{Some SIRS-type  epidemic models}\lab{s:SIR}
We start by providing a simple SIRS model, which includes however several ``non-classic" interesting interactions, like loss of immunity and vaccination.

% (inspired by the classical SIR model) with constant vaccination and logistic growth of \cite{Rodrigues}:}  %~\cite{Makinde2007,Shulgin1998,Stone2000}.
 \usetikzlibrary{arrows,positioning}
\begin{center}
\begin{figure}[H]
\begin{tikzpicture}%[scale=0.80]
[
auto,
>=latex',
every node/.append style={align=center},
int/.style={draw, minimum size=1.75cm}
]

    \node [fill=lightgray,int] (S)             {  $S$};
    \node [fill=lightgray,int, right=5cm] (I) {  $I$};
    \node [fill=lightgray,int, right=11cm] (R) {  $R$};

    \node [below=of S] (s) {} ;
    \node [below=of I] (i) {} ;
    \node [below=of R] (r) {};

    \node [above=of S] (os) {};
    \node [above=of I] (oi) {};
    \node [above=of R] (or) {};

    \coordinate[right=of I] (out);
    \path[->, auto=false,line width=0.35mm]
    			(S) edge node {$\beta I S$ \\[.6em]} (I)
                          (I) edge node {$\gamma _i I %/(1+\epsilon I)
                          $       \\[.6em] } (R) ;

 \path[->, auto=false,line width=0.35mm]
			(S) edge  [out=-120, in=-60] node[below] {$\lambda - \mu S$ \\ [0.2em] \emph{Constant growth}} (S)
    			(I) (5.88,-0.87cm) edge [] node[right]{$\mu _i I=(\mu + \de) I$} (5.88,-2cm) (i)
    			(R) (11.88,-0.87cm) edge [] node[right]{$\mu R$} (11.88,-2cm) (r) ;
			
    \path[-, auto=false,line width=0.35mm]
    			(S) (0,0.87cm) edge [] node[right]{} (0,2cm) (os)
			(os) (0,2cm) edge [] node[above]{$\gamma _s S$} (11.88,2cm) (or)
			(or) (11.88,2cm) edge [->] node[below]{} (11.88,0.87cm) (R) ;
    \path[-, auto=false,line width=0.35mm]
    			(S) (-0.5,0.87cm) edge [<-] node[right]{} (-0.5,2.5cm) (os)
			(os) (-0.5,2.5cm) edge [] node[above]{$\gamma _r R$} (12.3,2.5cm) (or)
			(or) (12.3,2.5cm) edge [] node[below]{} (12.3,0.87cm) (R) ;

\end{tikzpicture}
\caption{\small Illustration of the interaction between the classes of \emph{Susceptible}, \emph{Infectious} and \emph{Recovered} individuals in the SIR model $
\bep
\s' \\\iem  ' \\\r' \eep =  \bep \lambda- \b \s  \iem   -(\g_s+\mu) \s +\gamma_r \r   \\
 \iem  \pp{ \b \s    -(\gamma _i+\mu +\delta) } \\
\gamma _i \iem   -(\gamma_r +\mu)\r  +\g_s \s
\eep.
$
 Boxes represent compartments, and arrows indicate the flow between compartments.}
\label{boxes}
\end{figure}
\end{center}

\beD \lab{d:inf} a) For  an essentially nonnegative ODE defined on the nonnegative cone which admits some boundary fixed point $X_b$, let $X=(x,y)$ be the partition of the coordinates into the support $y=\{j:X_j>0\}$ and the set $x$ of coordinates which become $0$ at $X=X_b$.  The coordinates $y$ are also called resident in ME, and the coordinates $x$ are  called invading/infection. The equations for $x'$ are called infection equations (note, {\bf for polynomial systems}, that they may be written as $x'=A(x) x$.

b) We define the new infection terms to be {\bf all} the  nonlinear terms in the infection  equations which are also positive.

c) The new infection matrix $F$ is the matrix containing {\bf all} the new infection terms, and the matrix $V$ is defined by $j_I=F-V$, where $j_I$ is the derivative of the infection equations with respect to the infection variables.



d)  $R_0$ of the ODE at $X_b$ is the spectral radius (and Perron-Frobenius eigenvalue) of the matrix ${K =} F V^{-1},$ i.e.
$$R_0=R_0(F,V)=\lambda_{PF}(K)=\lambda_{PF}(F V^{-1}).$$
\eeD

\beXa The example in  figure \ref{boxes} admits one boundary point, $X_{dfe}=\pr{\sd=\frac{\lambda  \left(\mu +\gamma _r\right)}{\mu  \left(\mu +\gamma _r+\gamma _s\right)},
0,\rd=\frac{\lambda  \gamma _s}{\mu  \left(\mu +\gamma _r+\gamma _s\right)}},$  the new infection term is $ F=  \sd \beta,$
and  the derivative of the infection equation $i'$ with respect to the infection variable $i$ yields $ V=  \mu+\delta+\gamma_i.  $
Thus, $K= \sd \beta \frac{1}{\mu+\gamma_i+\delta}:= R_0.$
\eeXa

\beR The result of \cite{Diek,Van,Van08} is  that the inequality $R_0(F,V)<1$
determines correctly the domain of stability of $X_b$, 
provided a series of conditions are satisfied. They do not provide a unique choice of $F,V$, and indeed several choices \satg\ their conditions $F,V$ may be possible. 
 the word ``all new infection terms". 
 
 However, it was observed in many examples and hence conjectured in \cite{AABJ} that the ``all" choice satisfies always the conditions of \cite{Diek,Van,Van08}. Since our point of view here is algorithmic, like in  \cite{AABJ},  we make  the time-saving  choice of $F,V$ proposed in that paper. Note that it is an open problem to provide  a counterexample where the ``all" choice doesn't \saty\  the conditions of \cite{Diek,Van,Van08}.
 
 

  Finally, note that the unique choice made in definition \ref{d:inf} b),c) is not strictly necessary, since  different expressions for  $R_0$'s may  lead to the same domain of stability.


 


\eeR
%\beR An example of how  definition \ref{d:inf} a) applies is provided in section \ref{s:EnvZ}.




\subsection{Epidemic models  are formally CRNs}\label{s:SIRCRN}
Here is a three species,  eight
 ``directions/reactions" CRN representations of
the SIRS from Figure \ref{boxes}:
 {
   \begin{gather}\label{SIRS}
 x'=\bep
\s' \\\iem  ' \\\r' \eep =  \bep 1&- 1&0&1&-1&-1&0&0 \\
  0&1&- 1&0&0&0&-1&0\\
  0&0&1&- 1&1&0&0&-1
\eep \bep\lambda\\
\b \s  \iem   \\ \g_i \iem   \\ \g_r \r \\ \g_s \s \\\mu \s \\(\mu+\de)\iem   \\ \mu \r \eep =\Gamma \bf R(x).
\end{gather}

}
{
Here  $ \bf R(x)$ is the vector of rates of change in each direction, for example $\lambda$ acts on $\s$ only, and
$\Gamma$,  the ``directions/stoichiometric matrix", has columns which  give the respective directions in which each rate acts. Identifying the stoichiometric matrix allows computing CRN theoretical quantities like the deficiency (a measure of the complexity), which is 1, the conservations  space (i.e. the maximal non-negative cone included in  the kernel/nullspace to the left), and the elementary generators (i.e. a basis for non-negative vectors which are orthogonal to $\G$ from the right).

\beR \lab{r:SIRa}We can also represent the model via its eight reactions
RN=\{$0\to "S","S"+"I"\to 2 "I","I"\to "R","R"\to "S","S"\to "R","S"\to 0,"I"\to 0,"R"\to 0$\} (note the second reaction, which makes the model  {\bf explicitly/one step autocatalytic}, since $I$ appears on both sides of the reaction, and renders results which assert that  bifurcations  exist a priori if the kinetics is ``rich  enough" (for example Michaelis-Menten)   to be expected  \cite{Vas,VasStad}).

The  ``\HJF"  graph having the complexes as vertices and reactions as edges is displayed in the following figure:
\figu{SIRSgr1}{The FHJ graph of the ``SIRS network" with $8$ reactions and the deficiency $\de=6-2-3=1$. The $0$ node represents the exterior.}{.9}
\eeR
%SIRS.nb
%Graphs-RN.nb

\subsection{The mass-action SIRS has a unique, rational endemic point  when $R_0 >1$, which is globally asymptotically stable:  SIRS.nb (3,8,3,1)}\label{s:SIRS}

We recall here the fact that SIRS has a quite simple dynamic landscape:
\BEN \im  One boundary \DFE\ (DFE) fixed point
$$(\sd=\frac{\lambda  \left(\mu +\gamma _r\right)}{\mu  \left(\mu +\gamma _r+\gamma _s\right)}, 0, \rd=\frac{\lambda  \gamma _s}{\mu  \left(\mu +\gamma _r+\gamma _s\right)}).$$
\beR
The stability condition of the DFE may  be expressed as  the product
$$R_0:=\sd \frac{  \beta  }{ \gamma_i +\mu _i}:=\sd \mR <1, $$
where $\mR$ is a measure of the "number of infections produced by one infectious individual". In general, $R_0$ is the spectral radius of the "\NGM" \cite{Diek,Van,Van08}.
\eeR
\im   One rational  endemic point given by
\begin{flalign*}
\mbox{EE}=  \pr{\frac{\gamma_i +\mu _i}{\beta }:=\fr 1{\mR}, \frac{\mu  \left(\gamma_i +\mu _i\right)
  \left(\mu +\gamma _r+\gamma _s\right)(R_0-1)}{\beta  \gamma_i  \mu +\beta  \mu _i \left(\mu +\gamma _r\right)}, \frac{\beta  \gamma_i  \lambda -\left(\gamma_i +\mu _i\right)
  \left(\gamma_i  \mu -\mu _i \gamma _s\right)}{\beta  \gamma_i  \mu +\beta  \mu _i \left(\mu +\gamma _r\right)}},
\end{flalign*}
where $\mu_i=\delta+\mu$.
The existence of just one rational endemic point is discovered here by
\lstinline[language=Mathematica]{Solve[RHS==0,var]}
(in cases where the execution ``hangs", we will know that the fixed points are not all rational, and a different approach, a rational univariate representation (RUR) may be used).
\beR
As is often the case  in simple ME models, the $i$ component of the endemic \fp\ becomes positive and stable precisely when
\be{R0frS} R_0=\sd \mR=\fr{\sd}{s_e}>1,\ee
and at $R_0=1$ it equals the DFE.  Thus, we have here a ``relay phenomena": precisely when the DFE loses stability, a new fixed point enters the domain,  and  takes over.
\eeR
\im    The local stability  of the  endemic  fixed  point when $R_0>1$ is checked via Routh-Hurwitz criterion in only $1$sec when $\gamma_s=0$; the same computation took  $64 $sec when $\gamma_s>0$ --See [SIRS.nb].

\im  Global asymptotic stability of the EE when it exists was established in \cite{BaiSIRSglob,EricAngGlob}.
\EEN

\beR There exist probably no ME models with  deficiency zero (in the weakly reversible case, they would be counterexamples to the global attractor conjecture, and for the weakly reversible case see \cite[Remark 6.1.B]{Fei87}).\eeR
\beO Analyze the stability of SIRS %and the SEIR of \cite{LiGraef}
using deficiency one theory. \eeO



==> SIRn.tex <==
\section{A challenge problem: the SIRnS  cyclic epidemic model with one susceptible class, one infection class,  and $n$ recovered classes}\lab{s:SIRn}
{
In this section, we present the  SIRnS epidemic model  for the evolution of susceptibles, infectives and recovered with several stages $s,i,r_1,...,r_n$, among a   population which increases  by a  constant birth (or immigration)  rate $\l$, and decreases via natural deaths only:
  \be{SIRn} \bc s'=\l -\b s i - \mu s -\g_s  s +\g_n r_n\\
i'=i\pr{\b s  + \sum_{k=1}^n \b_k   r_k  -\g  -\mu_i }
\\r_1'=\g i - r_1\pr{\b_1    i+ \g_1   + \mu_1 }\\ \vdots \\
r_{k}'=\g_{k-1} r_{k-1} - r_{k}\pr{\b_{k}    i + \g_k + \mu_k   }, k=2,\dots,n-1 \\
r_{n}'=\g_{n-1} r_{n-1} - r_{n}\pr{\b_{n}    i + \g_n + \mu_n   }+\g_s  s\ec.\ee

\beR  When $n=1$ and $\b_1=0$, SIRnS reduces to the SIRS model, and when $n=1$ and $\b_1= \g_1=0$, it reduces to the SIR model.
\eeR

It is easy to show that the unique boundary point is:
$\sd= \frac{\lambda }{\mu+\g_s },i=r_1=r_2=...=r_n=0, R_0=\sd \frac{\beta   }{\gamma +\mu }.$


\beR When $\mu=\mu_{1}...\mu_{n}$, let $N=N_t=s+ i +\sum_{k=1}^n    r_k$, and  note that $N'=\l - \mu N$ (all the other terms cancel), and that $N_0=\fr \l \mu  \Lra N_t=\fr \l \mu , \for t \ge 0$; in this case, dimension reduction is possible using  $s+ i +\sum_{k=1}^n    r_k=\fr \l \mu$, if so desired.

\eeR

{\bf Assumption}: Epidemiological considerations  advocate imposing the following constraints on the
constants $\b_k$
\be{bcon} 0 \leq \beta_1\leq \beta_{2}\leq...\leq\beta_n \leq \beta.\ee

To conform to the classic interpretation of recovered being fully non-infective,  we  may assume also $\b_1=0$.

\beR  There is no known virus for which \eqr{bcon} doesn't hold.  Nevertheless, the case of  "perverse viruses" (maybe with the opposite inequalities holding) deserves to be studied as well.\eeR


\beR The model \eqr{SIRn} above is motivated by several papers of Hethcote, starting with \cite[(4.1)]{HethSVDD}, where the case  $\beta_1=...=\beta_n=0,
\g_1=...=\g_n, \lambda=\mu=\mu_{1}...\mu_{n}=0$ was considered.
The stochastic version of this is  a SIRS model without demography (this is not essential), in which the loss of immunity period is Erlang distributed. Variations of the model  have also been studied in the context of enzyme kinetics, under the name of Glass-Kauffman model \cite{swick1985some,zaslavsky1995stability}.

Subsequently,  \cite{Carlos}  proposed introducing the parameters $\b_k \geq 0$, which take into account the fact that during the    "Erlang stages of transition from $i$ to $s$ there should  be a gradual immunity  loss, and  increase of  infectiousness;  this renders the problem considerably more challenging, for example the uniqueness of the endemic fixed point may be lost (open problem).


One interesting aspect of the \cite{HethSVDD} model, where the endemic point is unique,  is the existence of  Hopf bifurcations, for $n\ge 3$ \cite[pg. 7]{HethSVDD}, which is
quite unusual for  models which have a unique rational endemic point.

The model \eqr{SIRn} above is considerably more sophisticated than \cite[(4.1)]{HethSVDD}.
Despite that, \cite{AAV} established the existence of  Hopf and zero eigenvalue bifurcations for this model, using the inheritance theorem of CRNT. Also, the
possible multi-stationarity was circumvented, by using a Jacobian parametrization in the style of Clarke \cite{Clarke}.

\eeR

%\beR \cite[Lemma 4.1]{HethSVDD} provides an integral representation for the periodic solutions of their model. \eeR



\beR From the point of view of CRNT, % with $\fr \l \mu =1$,
we have a bimolecular model  of type $(n+2,2(n+1)+1,n+2)$,  using the terminology of \cite{BanBor}, who classified all mass action
networks of  type (3,4,3) for the presence of Hopf bifurcations. So, our model is considerably harder, and only choosing all $\b_i=0$, when the model is of type $(n+2,n+3,n+2)$  gets us closer to the  setup of \cite{BanBor} (the particular   case $n=1$ was completely elucidated in that paper, and some results for the case $(n,n+1,n)$ were obtained as well).\eeR

}





==> ShiFei.tex <==
\subsection{The (5,6,3,1) IDHKP-IDH system~\cite{ShiFei,joshi2024bifunctional}: IDHKP.nb
 does not \saty\ the NGM conditions, but \sats\ \eqr{R0fr}}
 \lab{s:ShiFei}
The following (5,6,3,1) network
	 \begin{equation}\label{e.ptm}
	       \begin{tikzcd}
S_1 + C_0 \arrow[r,yshift=+0.5ex,"k_1"] & C_1 \arrow[l,yshift=-0.5ex,"k_2"] \arrow[r,yshift=+0.5ex,"k_3"]& S_2 + C_0 & \\
[-0.1in]
S_2 + C_1 \arrow[r,yshift=+0.5ex,"k_4"] & C_2 \arrow[l,yshift=-0.5ex,"k_{5}"] \arrow[r,yshift=+0.5ex,"k_{6}"]& S_1 + C_1 &
      \end{tikzcd}
%\begin{array}{rl}  S_1+ C_0\xrightleftharpoons[k_2]{k_1}
%C_1 \xrightarrow{k_3} S_2+C_0\\ S_2+C_1 \xrightleftharpoons[k_5]{k_4}
%C_2 \xrightarrow{k_6} S_1+C_1 \end{array}
\end{equation}
was introduced in \cite{ShiFei}, as an example of network satisfying the sufficient
ACR conditions of having deficiency one, and two non-terminal complexes
($C_1, S_2+C_1$), (the terminal complexes above are $(S_2+C_0, S_1+C_1$),
which
  differ in a single species).

	Denote the state vector by $x=[C_0,S_1,C_1,S_2,C_2]^T$. The corresponding ODE can be written as:
	 \begin{gather} \nonumber\dot x=\frac{d}{dt}\bep C_0\\S_1\\C_1\\S_2\\ C_2 \eep=
\left(
\begin{array}{cccccc}
 -1 & 1 & 1 & 0 & 0 & 0 \\
 -1 & 1 & 0 & 0 & 0 & 1 \\
 1 & -1 & -1 & -1 & 1 & 1 \\
 0 & 0 & 1 & -1 & 1 & 0 \\
 0 & 0 & 0 & 1 & -1 & -1 \\
\end{array}
\right)
\bep  k_1 C_0S_1\\C_1 k_2\\C_1 k_3\\C_1 k_4 S_2\\C_2 k_5\\C_2 k_6\eep =
 \\ \bc C_1 \left(k_2+k_3\right)- k_1 C_0S_1\\C_2 k_6-k_1 C_0S_1+C_1 k_2\\C_2 \left(k_5+k_6\right)+ k_1 C_0S-C_1 \left(k_4 S_2+k_2+k_3\right)\\C_2 k_5+C_1 \left(k_3-k_4 S_2\right)\\
C_1 k_4 S_2-C_2 \left(k_5+k_6\right)\ec
\end{gather}
\iffalse
{\bf The structure of the file IDHKP.nb}. We turn now to a topic important in scientific computing: fleshing out a programming structure which  depends the least possible on the particular example under study; this  is not enough discussed in neither the ME and CRN literatures, which often view each example as a new world, even though, as already noted by Guckenheimer, the similarity between small dimension examples  is that considerable, that a  common ``universal solver notebook'' might be conceivable.
\fi
\BEN \im The two conservation laws
\be{RAPc}\left(
\begin{array}{c}
 C_0+C_2+C_1 \\
 2 C_2+C_1+S_1+S_2 \\
\end{array}
\right)=\left(
\begin{array}{c} c_{tot}\\
s_{tot}\end{array}
\right)\ee
 imply that the network  admits
a conservation with all coefficients positive.


 \im Here again, Solve[RHS==0,var] finds quickly all the steady states, which include the following rational parametrization:
    \be{RAPi} \bc S_1= \frac{k_2+k_3}{ k_1}\frac{C_1}{C_0}\\
    S_2=  \frac{k_3 \left(k_5+k_6\right)}{k_4 k_6}
   \\ C_2= \frac{k_3}{k_6} C_1.\ec \ee
Note the second component identifies the ACR species (in agreement with the \cite{ShiFei} criterion), with ACR value $s_2^*=  \frac{k_3 \left(k_5+k_6\right)}{k_4 k_6}$.



This ODE has also one ``DFE''   fixed point
 \be{DFEs}S_1=0,S_2=s_{tot}, C_1=0,C_2=0, C_0=c_{tot} .\ee
   Indeed, setting $C_1=C_2=0 \Lra S_1=0$ or $C_0=0$;
the second case is impossible by the first equation in \eqr{RAPc},
and the first case yields the DFE. Therefore, the resident species are $\{C_0, S_2\}$ and the infectious species are $\{S_1, C_1, C_2\}$.


\im Next, we turn to the NGM approach, which starts by splitting the RHS of the differential equations for the infectious species $S_1,C_1,C_2$ as follows
\begin{gather*}
\bep -C_0 k_1 S_1+C_1 k_2+C_2 k_6\\C_0 k_1 S_1-C_1 \left(k_4 S_2+k_2+k_3\right)+C_2 \left(k_5+k_6\right)\\C_1 k_4 S_2-C_2 \left(k_5+k_6\right)\eep=\mF-\mV\\:=
\bep 0\\
C_0 k_1 S_1
\\C_1 k_4 S_2\eep-
\bep C_0 k_1 S_1-C_1 k_2-C_2 k_6\\
C_1 \left(k_4 S_2+k_2+k_3\right)-C_2 \left(k_5+k_6\right)
\\C_2 \left(k_5+k_6\right)\eep
\end{gather*}
(the  ``new infections'' part $\mF$  contains only nonlinear, positive interactions, and $\mV$ must have must have  nonnegative  sum, which is not \satd\ here, since the sum is $-C_2 k_6$.
\im  We turn therefore to classic stability analysis. The \ch\ of the full Jacobian
 factors out $u^2$. The resulting third order polynomial (note that we have reduced
 the dimension without using the  NGM theorem)  further simplifies at the DFE to a polynomial for which  only the  first coefficient may change sign, and this happens at $s_2^*=s_{tot}$.

 \im  Despite the fact that in this example the condition (A4) of the NGM theorem \cite{Van08} isn't satisfied, we have used  the ``NGM heuristic", which gets here the correct  stability domain of the DFE. Decomposing the Jacobian of the  infection  equations \wrt\ the  infection  variables as
 \begin{gather*} \lab{Gr} Gr=\left(
\begin{array}{ccccc}
 -k_1 C_0& k_2 & k_6 \\
 k_1 C_0& -k_4 S_2-k_2-k_3 & k_5+k_6 \\
 0 & k_4 S_2 & -k_5-k_6 \\
\end{array}
\right)=F-V, \\F=\left(
\begin{array}{ccccc}
 0 & 0 & 0 \\
 k_1 C_0& 0 & 0 \\
 0 & {k_4 S_2} & 0 \\
\end{array}
\right),-V=\left(
\begin{array}{ccccccc}
 -k_1 C_0& k_2 & k_6 \\
 0& -k_4 S_2-k_2-k_3 & k_5+k_6 \\
 0 & 0 & -k_5-k_6
\end{array}
\right)
\end{gather*}
yields a \NGM\ with one zero \eig\ and one complicated $R_0$ given by a quadratic formula. Reducing $R_0<1$ may be done by Mathematica; alternatively, the substitution $u\to x+1$ yields a second order polynomial where only the free \coe\ $k_3 \left(k_5+k_6\right)-k_4 k_6 s_{tot}$ may change sign, and the RH criterion yields
 that stability of the DFE occurs when \be{RH2}\frac{k_3 (k_5+k_6)}{k_4 k_6} > s_{tot}\ee
 i.e. when the ACR value is outside the domain. Note that this of the form satisfies \eqr{R0fr}.



 \im It may be shown further by CAS analysis that, besides the DFE, each conservation class may contain
  a   second  fixed point  ``EE'', \satg\ \eqr{RAPi},
 which has all coordinates positive,  when
 \be{cin} \frac{k_3 \left(k_5+k_6\right)}{k_4 k_6} \leq s_{tot},\ee
which is precisely the complement of the condition \eqr{RH2}, and that the non-boundary steady state is stable whenever it exists.

\EEN

\beCo We conjecture
that  the EE  is globally asymptotically  stable
  when  \eqr{cin} holds.\eeCo
   Note that the problem of global dynamical properties of ACR networks,
  called {\bf dynamic ACR}, was only recently studied in \cite{joshi-craciun-2},
  for two reactions and two species.








==> Sircap.tex <==
\subsection{An example of ``symbolic/structural  Hopf bifurcation": the  Capasso-type SIRS model with  one functional infection rate: SIRSCap.nb}\lab{s:SIRScap}

We have seen in the previous section that the mass-action SIRS-type  epidemic model does not admit Hopf bifurcations. Here, we show that replacing mass-action kinetics with more general nonlinear interactions gives rise to the possibility of purely imaginary eigenvalues crossings (recall that this is always true with two functional  rates, infection and treatment \cite[Thm 3.1]{AAV}). Furthermore, an example may be detected simply by Mathematica's command FindInstance.

 The Capasso-type SIR model   \cite{Capasso}  we consider is:
 \begin{gather}\label{Cap}
\nonumber\bep s'\\i'\\r' \eep
=\left(
\begin{array}{ccccc}
 \lambda  & -1 & -\mu -\gamma _s & 0 & \gamma _r \\
 0 & 1 & 0 & -\gamma -\mu _i & 0 \\
 0 & 0 & \gamma _s & \gamma  & -\mu -\gamma _r \\
\end{array}
\right) \bep 1\\ i s f(i)\\ s\\ i\\ r \eep \\ 
=\bep \lambda -i s f(i)- s (\mu+\gamma_s) + r  \g_r\\
i s f(i)-i \left(\gamma +\mu _i\right)\\
\gamma  i-r (\mu+\gamma_r)+ s \g_s
\eep
\end{gather}


The flux balance (fixed point) equations -- see SIRSCap.nb -- impose three conditions:
$$\bc \lambda = \frac{i f(i) \left(\gamma  \mu +\mu _i \left(\mu +\gamma _r\right)\right)+\mu  \left(\gamma +\mu _i\right) \left(\mu +\gamma _r+\gamma _s\right)}{f(i) \left(\mu +\gamma _r\right)}\\s= \frac{\gamma +\mu _i}{f(i)}\\r= \frac{\gamma  i f(i)+\gamma _s \left(\gamma +\mu _i\right)}{f(i) \left(\mu +\gamma _r\right)}\ec$$

The Hopf condition \be{H3} H_3:=co_2 co_3-co_1 co_4=0,\ee where $co_i$ are the coefficients  on the \ch\ of the Jacobian at equilibrium (with $\l, s, r$ eliminated):
$$jac=\left(
\begin{array}{ccc}
 -i f(i)-\mu -\gamma _s & -\gamma +\frac{i f'(i) \left(-\gamma -\mu _i\right)}{f(i)}-\mu _i & \gamma _r \\
 i f(i) & \frac{i f'(i) \left(\gamma +\mu _i\right)}{f(i)} & 0 \\
 \gamma _s & \gamma  & -\mu -\gamma _r \\
\end{array}
\right)$$
imposes  an extra condition on $f'(i)$. Finally, looking for an example  with FindInstance which
satisfies also the positivity conditions yields
\bea && i= 1,\gamma = 2,\gamma _r= 1,\gamma _s= \frac{1}{2},\mu = \frac{1}{128},\mu _i= 1,f(i)= \frac{7}{32}\\ \Lra
&& \lambda = \frac{4247}{3612},s= \frac{96}{7},r= \frac{7936}{903}, f'(i) = \frac{7}{291} \left(\frac{7179}{2048}-\frac{\sqrt{72187889}}{4096}\right) >0 .
\eea
As a check, the resulting Jacobian has eigenvalues $-1.26227,  0.415878 I,  - 0.415878 I$.

As for parametric conditions on $f(i), f'(i)$, they can often be satisfied with enough parameters \cite{Vas}. For example, the instance above with \MM| infection rate $f(i)=\fr \b{1 + \ep i}$,
yields $$\beta= \frac{24 \left(\sqrt{72187889}+51606\right)}{3815893},\epsilon=\frac{768 \sqrt{72187889}+12922157}{26711251}$$





\iffalse
\blue{and by assuming $\mu_i=\mu$ , we find that the first coefficients of the quadratic polynomial corresponding to the Jacobian   are
\bea
\bc
\frac{\mu  \left(i^2 \epsilon  \left(\beta  \left(\gamma +\mu +\gamma _r\right)+\epsilon  (\gamma +\mu ) \left(\mu +\gamma _r+\gamma _s\right)\right)+i \left(\beta  \left(\gamma +\mu +\gamma _r\right)+2 \epsilon  (\gamma +\mu ) \left(\mu +\gamma _r+\gamma _s\right)\right)-\left(\mu +\gamma _r+\gamma _s\right) (-\gamma -\mu +\beta  s)\right)}{(i \epsilon +1)^2},\\
\frac{i^2 \epsilon  \left(\beta  \left(\gamma +2 \mu +\gamma _r\right)+\epsilon  \left(3 \mu ^2+2 \mu  \left(\gamma +\gamma _r+\gamma _s\right)+\gamma  \left(\gamma _r+\gamma _s\right)\right)\right)+i \left(\beta  \left(\gamma +2 \mu +\gamma _r\right)+2 \epsilon  \left(3 \mu ^2+2 \mu  \left(\gamma +\gamma _r+\gamma _s\right)+\gamma  \left(\gamma _r+\gamma _s\right)\right)\right)+3 \mu ^2-\beta  s \left(2 \mu +\gamma _r+\gamma _s\right)+2 \mu  \left(\gamma +\gamma _r+\gamma _s\right)+\gamma  \left(\gamma _r+\gamma _s\right)}{(i \epsilon +1)^2},\\
\gamma +\frac{\beta  \left(i^2 \epsilon +i-s\right)}{(i \epsilon +1)^2}+3 \mu +\gamma _r+\gamma _s,
\ec
\eea
which  yields to the Following Routh-Hurwitz function
\bea
&& \Scale[1]{h_3=\frac{1}{(i \epsilon +1)^4}\pr{\gamma +i^2 \epsilon  \left(\beta +\epsilon  \left(\gamma +2 \mu +\gamma _r+\gamma _s\right)\right)+i \left(\beta +2 \epsilon  \left(\gamma +2 \mu +\gamma _r+\gamma _s\right)\right)+2 \mu +\gamma _r-\beta  s+\gamma _s}}\\
&&\Scale[.9]{\pr{i^2 \epsilon  \left(\beta  \left(\gamma +2 \mu +\gamma _r\right)+\epsilon  (\gamma +2 \mu ) \left(2 \mu +\gamma _r+\gamma _s\right)\right)+i \left(\beta  \left(\gamma +2 \mu +\gamma _r\right)+2 \epsilon  (\gamma +2 \mu ) \left(2 \mu +\gamma _r+\gamma _s\right)\right)-\left(2 \mu +\gamma _r+\gamma _s\right) (-\gamma -2 \mu +\beta  s)}.}
\eea
The following instance ensures the positivity of the previous coefficients and satisfy $h_3=0$:
$$\pr{\gamma = 4,\gamma _r= 1,\mu = 1,\gamma _s= 1,i= \frac{5}{16},s= 1,\beta = \frac{3528}{151},\epsilon = 1}\Rightarrow f(i)=\frac{2688}{151}.$$
In that case, the eigenvalues of the Jacobian are given by $\pr{\pm 2.77286\; Im,-1},$ which   confirms the existence of Hopf. }





\purple{In the following, we use the substitution of the flux balance equations, and the \MM| infection rate $f(i)=\fr \b{1 + \ep i}$, we find  that in the simplified case $\mu_i=\mu$, the coefficicents of the characteristic polynomial corresponding to the Jacobian with monomial $1$ are positive and are given by
\bea
\bc
\frac{i \mu  \left(\beta  \left(\gamma +\mu +\gamma _r\right)+\epsilon  (\gamma +\mu ) \left(\mu +\gamma _r+\gamma _s\right)\right)}{i \epsilon +1}>0,\\
\frac{\beta  i \left(\gamma +2 \mu +\gamma _r\right)+i \epsilon  \left(3 \mu ^2+2 \mu  \left(\gamma +\gamma _r+\gamma _s\right)+\gamma  \left(\gamma _r+\gamma _s\right)\right)+\mu  \left(\mu +\gamma _r+\gamma _s\right)}{i \epsilon +1}>0,\\
\frac{i \left(\beta +\epsilon  \left(\gamma +3 \mu +\gamma _r+\gamma _s\right)\right)+2 \mu +\gamma _r+\gamma _s}{i \epsilon +1}>0.
\ec
\eea
Moreover, the Routh-Hurwitz criteria is
$$h_3=\frac{\left(\beta  i \left(\gamma +2 \mu +\gamma _r\right)+i \epsilon  (\gamma +2 \mu ) \left(2 \mu +\gamma _r+\gamma _s\right)+\mu  \left(2 \mu +\gamma _r+\gamma _s\right)\right) \left(i \left(\beta +\epsilon  \left(\gamma +2 \mu +\gamma _r+\gamma _s\right)\right)+\mu +\gamma _r+\gamma _s\right)}{(i \epsilon +1)^2}>0,$$
which precludes Hopf in that case. But when $\mu_i\neq \mu$, Mathematica fails to prove anything concerning Hopf.}
\fi

\beR The success  reported in this example hides the fact that the Mathematica execution time is quite sensitive to the parametrization. For example, using $ s f[i]$ instead of $i s f[i]$
in the parametrization of rates greatly increases  the execution time.  %For this reason, we will focus from now on more on systematic approaches developed in the CRN literature.
\eeR

%%%%%%%%%%%%%%%%
\iffalse
\blue{By computing the symbolic Jacobian of \eqr{Cap} and substituting $s=1-r-i$, we get}

$$ J=\left(
\begin{array}{ccc}
 -f(i) & (i+r-1) f'(i)+\mu _i & d_r \\
 f(i) & -\gamma -(i+r-1) f'(i)-\mu _i & 0 \\
 0 & \gamma  & -d_r \\
\end{array}
\right),$$


and then by implementing the following script into Mathematica, by using the function `\textbf{Hur3M}"
%we defined into our package `\textit{epid}",
 which compute the Routh Hurwitz criteria, as follows

\begin{verbatim}
{co, h3, ine} = Hur3M[jac];
{co0, co1, co2, co3} = co;
parc = Variables[co]; cp = Thread[parc > 0];
Timing[cH = FindInstance[Join[cp, {h3 == 0, eqS == 0}], parc][[1]]]
\end{verbatim}
\blue{where \textit{eqS} denotes  the sum of the second and third equations in \eqr{Cap} after substituting $s=1-i-r$, and it's given by
$$\text{eqS}=f(i) (1-i-r)-i \mu _i-r d_r,$$
the script yields
$$\pp{d_r= 1,i= \frac{5}{16},r= \frac{1}{2},\gamma = 1,\mu _i= 1,f(i)= \frac{13}{3},f'(i)= \frac{352}{9}}$$
and under this numerical instance, the eigenvalues of the Jacobian are $\pr{\pm 1.82574\; Im,0}.$}
\fi 


==> Ton1.tex <==

\subsection{The  (4,5,3,2) MAK with ACR   \cite[(1)]{tonello2018network} \sats\ $R_0={\fr{\sd}{s_e}}$: Tonello.nb}\lab{s:Ton}

We end this section by mentioning one idea which seems very important, in particular for the non-reversible models of ME. The reader may have noticed that one idea
of CRNT, the embedding of the \HJF\ into Euclidean space, does not seem fully exploited in classical CRNT, since it was not clear how moving the graph vertices around, and allowing them to collide, will affect the results. This implicit question has been now addressed in the theory of network translation, initiated by Johnston  \cite{John,tonello2018network,JMP,hernandez2022framework}, which examines among other things how network translation affects the \HJF\ graph structure.

 Network translation of a MAK to a ZD-WR GMAK helps understanding, among other things,  rational parametrizations related to the  matrix tree theorem (see for example \cite{CoxSl}) which appear in certain MAKs. Consider the MAK \cite[(1)]{tonello2018network} \begin{equation}\label{eq:proper_acr_intro}
      \begin{tikzcd}[row sep=small, column sep=small]
          & A + C & C \arrow[rd, "r_3"] & & \\
         A + B \arrow[ru, "r_1"] \arrow[rd, "r_2"'] & & & A \arrow[r, "r_5"] & B. \\
        & A + D & D \arrow[ru, "r_4"'] & &
      \end{tikzcd}
\end{equation}
with \sm\ $\left(
\begin{array}{ccccc}
 0 & 0 & 1 & 1 & -1 \\
 -1 & -1 & 0 & 0 & 1 \\
 1 & 0 & -1 & 0 & 0 \\
 0 & 1 & 0 & -1 & 0 \\
\end{array}
\right)$.

Ordering  the species (and the complexes) according to their appearance order yields the ODE: \beq &&\lab{ODET}\frac{d}{dt} \bep A\\
 B\\
 C\\
   D\eep=
   \bep-k_5 A+k_3 C+ k_4 D\\-A \left(k_1 B+k_2 B-k_5\right)\\
   k_1A B - k_3 C\\k_2A B - k_4 D\eep\eeq

\BEN \im
It can be checked that $rank(\Gamma)=3$, the deficiency is
$\delta=n_C-rank(\Gamma)-\ell=7-3-2=2,$
 the CRN has the conservation
$
A+B+C+D
$, and that the cone of positive fluxes has dimension 2.

 \im \Ma\ finds two fixed points
\be{Ton}\bc A= 0,B=n_{tot},C= 0,D= 0\\ B^*= \frac{k_5}{k_1+k_2},C= \frac{ k_1 k_5}{\left(k_1+k_2\right) k_3}A,D= \frac{ k_2 k_5}{\left(k_1+k_2\right) k_4}A\ec,\ee
which suggests that the \MTT\ might be at work.
The second solution under the extra constraint $A+B+C+D=n_{tot}$,
\[\bc A=\left(\left(k_1+k_2\right) n_{tot}-k_5\right)\frac{k_3 k_4 }{k_1 k_4 \left(k_3+k_5\right)+k_2 k_3 \left(k_4+k_5\right)},B^*= \frac{k_5}{k_1+k_2}\\C=\left(\left(k_1+k_2\right) n_{tot}-k_5\right)\frac{k_1 k_4 k_5 }{\left(k_1+k_2\right) \left(k_1 k_4 \left(k_3+k_5\right)+k_2 k_3 \left(k_4+k_5\right)\right)}\\D=\left(\left(k_1+k_2\right) n_{tot}-k_5\right)\frac{k_2 k_3 k_5 }{\left(k_1+k_2\right) \left(k_1 k_4 \left(k_3+k_5\right)+k_2 k_3 \left(k_4+k_5\right)\right)}\ec\] is
positive iff $n_{tot} >B^*$.
 %For the NGM method, we consider the ``rank 1'' matrices

  Let's consider the following decomposition of the infectious equations in \eqr{ODET} (produced by our NGM script from Epid-CRN):
  \iffalse
\[\blue{\mF-\mV = \bep k_3 C +k_4 D\\0\\0\eep -\bep k_5 A\\k_3 C-k_1 A B \\ k_4 D- k_2 A B \eep \Rightarrow } F=\left(
\begin{array}{ccccc}
 0 & k_3 & k_4 \\
 0 & 0 & 0 \\
 0 & 0 & 0 \\
\end{array}
\right),  V=\left(
\begin{array}{ccccccc}
 k_5 & 0 & 0 \\
 -k_1 B & k_3 & 0 \\
 -k_2 B & 0 & k_4
\end{array}
\right),\]
\blue{from the previous decomposition note that $\sum \mV_i=k_5 A + k_3 C+k_4 D- A B(k_1+k_2)$ which doesn't satisfy the condition \cite[(A4)]{Van08}, so the NGM cannot be applied.}
\fi
{
\[\mF-\mV=\bep 0\\ k_1 A B\\ k_2 A B\eep -\bep k_5 A-k_3 C -k_4 D\\ k_3 C\\ k_4 D\eep\]
The condition \cite[(A4)]{Van08} is satisfied  since $\sum \mV=k_5 A >0$ (and all the other conditions are \satd\ as well). Now
\[F=\left(
\begin{array}{ccc}
 0 & 0 & 0 \\
 B k_1 & 0 & 0 \\
 B k_2 & 0 & 0 \\
\end{array}
\right), V= \left(
\begin{array}{ccc}
 k_5 & -k_3 & -k_4 \\
 0 & k_3 & 0 \\
 0 & 0 & k_4 \\
\end{array}
\right)\Rightarrow K=\left(
\begin{array}{ccc}
 0 & 0 & 0 \\
 \frac{B k_1}{k_5} & \frac{B k_1}{k_5} & \frac{B k_1}{k_5} \\
 \frac{B k_2}{k_5} & \frac{B k_2}{k_5} & \frac{B k_2}{k_5} \\
\end{array}
\right).\]
The cubic \ch\ of $K$ is $\mbox{ch}(u)=\frac{u^2 \left(n_{tot} (k_1+ k_2)-k_5 u\right)}{k_5}$. After
removing the factor $u^2$, the remaining first order polynomial has one positive root $\fr{n_{tot}}{B^*}$
implying that the DFE is stable iff $R_0:=\fr{n_{tot}}{B^*} \leq 1$. }
%This yields $R_0=\fr{n_{tot}}{B^*}$,
Also, the Jacobian at the EE reveals that it is always stable, when  $R_0>1$.
\EEN
\iffalse
To better understand this model, the authors propose studying in parallel the GMAK
\begin{equation}\label{eq:proper_acr_intro_translated}
      \begin{tikzcd}[row sep=small, column sep=small]
        & & \mbox{\ovalbox{$\begin{array}{c} A+C \\ (C) \end{array}$}} \arrow[rd, "\tilde{r}_3"] & & & \\
& \mbox{\ovalbox{$\begin{array}{c} A+B \\ (A+B) \end{array}$}} \arrow[ru, "\tilde{r}_1"] \arrow[rd, "\tilde{r}_2"'] & & \mbox{\ovalbox{$\begin{array}{c} 2A \\ (A) \end{array}$}}. \arrow[ll, "\tilde{r}_5"] \\
        & & \mbox{\ovalbox{$\begin{array}{c} A+D \\ (D) \end{array}$}} \arrow[ru, "\tilde{r}_4"'] & & &
      \end{tikzcd}
    \end{equation}
    In \eqref{eq:proper_acr_intro_translated}, the lower (kinetic) complexes, displayed in parenthesis,  correspond to the original source complexes \citep{John}, and the upper (stoichiometric) complexes correspond to the source complexes adjusted by  ``translation complexes" (in this case,   $A$ was added to $r_3$, $r_4$, and $r_5$), with the net result of gluing some of the product complexes to source ones, and create this way a WR GMAK.

    Now the translated CRN, which represents the same dynamics, has ZD, and hence the \fp\ formulas may be interpreted via the \MTT, applied to the graph \eqref{eq:proper_acr_intro_translated} \cite[Thm 2-3]{tonello2018network}.

\fi




==> cat.tex <==
\section{A non-catalytic monomolecular translated SIRS model}\lab{s:cat}
As noted in Remark \ref{r:SIRa}, the presence of
$"S"+"I"\to 2 "I"$ in the reactions representation  makes the model  {\bf explicitly autocatalytic}, since $I$ appears on both sides of the reaction. We turn now to a variant of SIRS which is non-catalytic.
\beXa [A non-catalytic reversible monomolecular model with deficiency zero] \lab{e:linSIRS}
Consider now a ``monomolecular version", obtained by ``simplifying/translating" the second reaction "S"+"I"$\to$ 2 "I" to "S"$\to$ "I" \cite{John}.
\figu{SIRSlin}{The  ``monomolecular SIRS" has one linkage class, is   weakly reversible (WR), and has zero deficiency (ZD) 4-3-1=0.}{.8}


This process  has a unique globally attractive fixed point, which is positive for all values of the parameters. In fact, this is conjectured to hold always for the class of weakly reversible, zero deficiency (WR-ZD) CRNs by the so-called ``Global Attractor
Conjecture" \cite{horn1972general,CF05,CF06}, and is proved to hold ``robustly", for any admissible rate $r_1(s)$ in \cite[Sec.6,Exa 1]{ARS24} (however,  this simplified   model does not make  sense epidemiologically).
\eeXa

\beR This example reveals one possible interest  of the CRN-ME collaboration. ME models display often multi-stability and oscillations (which are always proved by example dependent methods). On the other hand, they  have typically   ``WR-ZD cousins", obtained by translation,  which are super well-behaved, and which may be obtained by off shelf software (involving sometimes Linear Programming) \cite{Hong}.

It is conceivable that the well-behaved cousins can help in reaching interesting conclusions for their more complex relatives, but this remains to be seen.
\eeR

\ssec{Non-catalytic and auto-catalytic CRNs may be defined based only on the SM and on the functional dependence in the rates}
\beR The definition of catalyticity below, due to A. Angeli, E.Sontag and  collaborators,  depart from the traditional one, which involves decomposing
the SM as the difference of an output SM and an input SM.
\eeR

\beD
The pattern of signs in $\G$ may be used to define a partition of {\bf each column   $\Gamma_i$} into \BEN \im the \textbf{products} of the reaction, corresponding to positive entries, and \im  \textbf{reactants}, corresponding to  negative entries.
\EEN
\eeD
\beD \lab{d:aut} A. A  CRN (see Definition \ref{d:R}) is {\bf non-catalytic} iff the variables  of all the reaction rates $R_j$
    are precisely the reactants, i.e. the species $i$ such that $ \G_{ij}< 0 $.

B.  A  CRN is {\bf auto-catalytic} if it is not non-catalytic, i.e. iff there exists some reaction rate $R_j$ whose arguments
    include  some species $i$ such that $ \G_{ij}> 0 $.
    \eeD

    \beR  \lab{r:adm} For a  \nc, or {\bf reactant-dependent} BIN/CRN, the rates must satisfy
\begin{enumerate}
 		\item[\bf A1.] $R_j(x)$ is continuously differentiable, $j=1,..,n_r$;
 		\item[\bf A2.] if $ \G_{ij}< 0$, then $x_i=0$ implies  $R_j(x)=0$; %
 		\item[\bf A3.] ${\partial R_j}/{\partial x_i}(x) \ge 0$ if $ \G_{ij}< 0$ and ${\partial R_j}/{\partial x_i}(x)\equiv 0$ if $ \G_{ij}\ge 0$;
 		%
 		%
 		%
 		\item[\bf A4.] The inequality in   {A3} holds strictly for all positive concentrations, i.e when $x \in \mathbb R_+^n$.
 		%
 	\end{enumerate}
 	\eeR 

==> cont.tex <==
\ssec{Contents} Since this essay is in part a notebook accompanied manual
for solving ME and CRN problems, one  issue  we encountered was ordering the problems by their complexity.
For that, we found useful  the CRN classification of complexity in \cite{BaBo23}, according to $(n_{Species}, n_{Reactions},rank)$, but we added at the end the deficiency.
\beD  The deficiency of a CRN is defined to be the number of complexes $|\mathcal{C}|$ minus the rank of the \sm, and minus the number of components in the \HJF\ graph (for further information on the deficiency theorems and CRN's in general, see for example the tutorials \cite{Gun,Ang,Yu,Cox}).
\eeD

 We  start in section \ref{s:SIR} with  some simple versions of the SIR model, included with the purpose of disseminating the basics of ME.
Section \ref{s:SIRS} provides a  notebook for a mass-action three species, eight reactions SIRS model, where the application of a Routh Hurwitz -type criterion for the unique positive endemic point is straightforward, and rules out Hopf bifurcations.
The notebook for section \ref{s:SIRScap} offers an example  with Hopf bifurcation
 for a SIRS model with one functional rate $f(i)$, in terms of the values $f(i), f'(i)$ at the endemic point. The example may be realized by choosing a Michaelis-Menten  type $f(i)$.

Section \ref{s:cat} takes a short detour through the world of non-catalytic CRNs, exemplified by a ''monomolecular translated SIRS model". This draws attention to the fact that while epidemic models are
auto-catalytic, they have non-catalytic relatives which might turn out useful in analyzing them.



 In section \ref{s:ACR} we turn to studying the stability  of CRN models displaying absolute concentration robustness (ACR)-- see Definition \ref{d:ACR}, via the \NGM\ (NGM) method.
  %{s:SIRSrob} lists results obtained with a Matlab LEARN notebook, for a robust SIRS model with no demography.



The initiation to ME models continues in section \ref{s:SIRn}, where we recall a  challenging mass-action model  SIRnS
 with $n+2$ compartments, first introduced in \cite{Carlos}, and further analyzed in \cite{AAV}. We   resolve in section \red{\ref{s:SIR1S}} one outstanding question,
 concerning  the existence of \Hb\ for   SIR1S (with n=1). %This was challenging for us computationally,  since SIR1S may have two non- rational fixed points, and required some care in choosing  the variables with respect to which we solved the fixed point + RH system.

\iffalse
Section \ref{s:Bulh} is included for three purposes:
\BEN \im  Firstly,  to  inform CRN researchers   on a quite complex two strains model  \cite{Bulh} -- see also \cite{AABJ},
which is appropriate for modelling the recurrent Dengue and Zika epidemics, and takes into account  both the antibody-dependent enhancement
(ADE) effect, and   the impact of vaccination applied to one strain only.
 \im Secondly, to draw attention to the interesting feature  that $R_0$ is the maximum of rational ``invasion  numbers'' related to the individual strains.
 It was noted in \cite{AABJ} that this simple structure is an outcome of the fact that the \ch\ of the Jacobian of the ``infection equations'' \wrt\ the ``infection variables''
 factors as a product of linear terms. This linear factorization property simplifies considerably the \RH\ criteria, and is clearly of interest to both communities.

\im \blue{Last but not least, we discuss in that section several natural questions surrounding the NGM approach. For readers which
encounter this for the first time, we mention that roughly, NGM is a  reduction method  for studying the stability of a boundary point, by looking only at the equations and variables
for the ``invading species'', i.e. the species which are  zero at the respective boundary point. \Fr it has been observed that in very complex symbolic models,
in which it  fails, sometimes further reductions are possible,
for example by factorizing a \ch, as noted already in \cite{AABJ}. While no theory concerning such factorizations seems to be available currently, it is definitely
worthwhile trying to understand them via examples.}
a
 %which include nonlinear terms .
  %and also a determination of domains of persistence and of global stability for the endemic point.
\EEN

 In section \ref{s:pho} we revisit some classic \RH\ analyses of mass action  phosphorylation models, which is one of the most extensively studied subfields of CRN.
 In section \ref{s:CMS}, we offer a Mathematica notebook and review
  of a famous  paper \cite{CMS}, which showed  the existence of Hopf bifurcations for a nine variables mass-action ``mixed phosphorylation'' model. Note that  the lack of Hopf bifurcations for 1-site
  phosphorylation was established also by robust methods in \cite{AAScomp}. \red{We complete the analysis of \cite{CMS} by showing precisely which of the additional reactions they considered introduced the Hopf bifurcations}.
%\EEN




 %The open problem of stability of  SEIRS/SAIRS type   modelsis revisited in section \ref{s:SAIR}. \red{...}

%In the ArXiv version,   we  review  also  some of the  robust Lyapunov function theory behind the package LEARN.
% illustrate them  in Mathematica notebooks associated to sections \ref{s:AAnew}, \ref{s:AAScomp}, ...
%Further examples illustrating the theory of k-contraction and usage of the package LEARN are provided in  section \ref{s:LEARN}.

Finally, in two last sections %\ref{s:CTMC}, \ref{s:esc},
included only in the ArXiv version, we draw the attention to similar, but harder problems concerning escape paths of stochastic CTMC extensions of our models.
\fi

==> res.tex <==
\ssec{Can CRN software solve ME problems?}\lab{s:res}
In this essay, we argued the case that ME researchers
 could profit from mastering the unifying language of biological interaction networks (BIN), or, under its more traditional name, chemical reaction networks (CRN) theory.  This language  is not used  in ME, despite the fact that  ME and BIN/CRN problems  are practically indistinguishable mathematically at first sight. As a result, ME researchers cannot profit from  the wealth of
   powerful CRN software, like for example \BEN \im
 The   collaborative package {CoNtRoL} (accessed on 6 August 2015) 
 \cite{donnell2014control,Control} \url{https://reaction-networks.net/wiki/CoNtRol}{;} 
 \im The  Mathematica packages ReactionKinetics \cite{Toth}, {MathCRN}  (accessed on 29 April 2016)
 \url{https://gitlab.com/csb.ethz/MathCrn} and
 reaction-networks.{m} \url{https://vcp.med.harvard.edu/software.html\#crnt};
 \im Feinberg's  Chemical Reaction networks {toolbox} \url{https://cbe.osu.edu/chemical-reaction-network-theory#toolbox};

 \im The Julia package Catalyst.jl \cite{catalyst};
 \im The Macaulay package ReactionNetworks.{m2} \url{https://macaulay2.com/doc/Macaulay2/share/doc/Macaulay2/ReactionNetworks/html/index.html};
  \im The  Matlab package {LEARN} \cite{AAnew,AAScomp,
Ali23gr} \url{https://github.com/malirdwi/LEARN}{;} 
\im The Matlab packages TowardZ and CASTANET for network translation, a topic initiated by {Johnston}  \cite{John,tonello2018network,JMP,hernandez2022framework}), implemented by {Hong et al.}  \url{ https://github.com/Mathbiomed/TOWARDZ} {and} 
 \url{https://github.com/Mathbiomed/CASTANET};
\im  The Python packages \cite{Tonello,crnpy} {and} 
 \url{https://github.com/materialsproject/reaction-network}.
\EEN

See {also}  
 \url{https://reaction-networks.net/wiki/Mathematics_of_Reaction_Networks} for further resources.

It is interesting to reflect on  the reason for the disparity between the strong computerization of CRN and its absence in ME for similarly looking problems. One reason is that ME strives towards complete analysis of small-dimension models (but see the 31 reactions model of \cite{Bulh} for an exception), {while CRN researchers study larger models but  settle  for partial answers (concerning, say, multistationarity and the existence of ACR) and avoid often difficult issues like the presence of Hopf and Bogdanov--Takens bifurcations, or chaos.}



Since ME models are formally CRNs, one can find out in two seconds what a CRN package like CoNtRoL has to say about the
simplest SIRS model: $S+I\to 2 I, I\to R\to S$. We receive lots of information; however, this does not  intersect a lot with what is considered important in ME about SIR,
which is:
\BEN \im  It admits only rational fixed points (which can be addressed via any symbolic  \CAS, without the need for special tools). \im It has only one interior fixed point if the crucial parameter $R_0$ determining the stability of the unique boundary fixed point is  fixed to be bigger than $1$.  The issue of possible ``phase transition constraints" on certain parameters  does  not seem to have been studied in CRN, where boundary fixed points have not been considered of much interest. \im  The ``endemic" interior fixed point previously mentioned is \GAS.
\EEN

It may be seen from the answers provided by CoNtRoL that the questions asked in ME and CRN are ``parallel, but not identical". % let us recall here just one famous open problem in CRN, the ``persistence conjecture"~\cite{Feinberg89}, which  asserts that a \emph{weakly-reversible} CRN must be persistent.  \Oth an ME model can never be persistent, since the DFE is locally attractive when $R_0 <1$ \cite{Diek,Van,Van08}.


\iffalse
These recent advances awaken the hope that one day in the future, the stability of small dynamical systems might be determined just by asking
ChatGPT or Alexa to check it (and they might  possibly consult surreptitiously Mathematica or Matlab dedicated programs before answering
--see opinion of  Stephen Wolfram \cite{wolfram2023chatgpt}).
\fi

Our paper has two motivations.
\BEN \im The first is to improve the communication between ME and CRN/BIN, by  informing the two communities about the  work of the other.
%ME theCRN/BIN methods, and by disseminating interesting open ME problems among CRN/BIN researchers.

For example, we bring to the attention of both communities open problems concerning a recent SIR-type model SIRnS \cite{Carlos,AAV}, which has $n+2$ \com s.

\iffalse
    CRN/BIN, which study more structured models,  have accumulated a rich body of results  for  specific  subclasses of ODE's, which have evolved into numeric computer packages like LEARN, able to deal sometimes with problems involving tens of variables.
In this essay, we are making the case that part of the
 methods (like for example
 results on k-contraction, robust stability and  robust non-oscillation) and packages  may be put to work for ME models.
\fi


\im
 A second   motivation is creating a package and disseminating example notebooks, whose tweaking might help solving new problems, as has long been standard in fields like  scientific computation and statistics.

  It seems fair to say  that until now, not enough effort has been invested in supporting ME papers by  scientific computing tools, despite the fact that a large number of ME papers  are dedicated to topics which are computational in essence (like computing stability and  bifurcation conditions).  For example, until our recent paper \cite{AABJ} and the package Epid-CRN, it was  impossible to find a symbolic script  which computes the famous epidemiology  stability  threshold $R_0$.

  \iffalse Typically,
ME researchers    exploit mostly example dependent computations  (often performed by  hand, which is occasionally indispensable in difficult cases), or  general purpose {\bf numerical} bifurcation packages.  As a justification for avoiding symbolic methods, it is often stated that the  symbolic Routh-Hurwicz (RH) stability conditions require too much computation time. This is definitely true,   but does not render the whole picture, given that there exist many flavours of RH, and also that CRN and algebraic geometry researchers (for example \cite{Gater}) manage to detect sometimes instabilities by using the  alternative ``{\bf reaction  coordinates}" \cite{Clarke}-- also see Remark \ref{r:reac}, or by graphical criteria, like for example the absence of critical siphons in Petri graphs (guaranteeing persistence), or by identifying instability producing subnetworks, called ``bad children" \cite{VasChild}.
\fi

We are introducing here the first version
of
our Mathematica computer package,  Epid-CRN, which integrates methods from both communities, and we accompany the paper by several pedagogic notebooks, dealing  mostly with classic examples from the literature. % for which notebooks areeither absent, or not in Mathematica, or less .
The novelty  are not the examples in themselves, but the fact that the solution is
structured in a way which strives to be independent of example, up to minor modifications.
Of course, the limits of our symbolic package are much lower than those of numeric packages; despite that, we hope our package will have at least a pedagogical value.

\EEN

Let us clarify here that the packages above already  achieve several of our goals. However, they are mainly geared to the CRN community, and  we hope that our package might  serve
 ME researchers as a  bridge towards  using CRN packages.  \Fr we hope to integrate
  methods not always available in  older packages, for example concerning injectivity \cite{CF05,BanPan},
monotonicity \cite{ADLS10gr,FWF17}, and persistence \cite{AdLSpetri}.\\
 %Among the notebooks provided to illustrate the   application of the package,
% we include some dedicated to the famous global stability versus Hopf bifurcation for SEIRS.


\iffalse
Before introducing our  package, which may be viewed also as a collection of ``stenographically convenient computational shortcuts", let us  warn the reader that the impressive LEARN is not immediately
applicable to ME models.
   The point is that while most of  the methods in LEARN   apply  to non-catalytic CRNs --see Definition \ref{d:aut},  ME models are autocatalytic, and the research of this class of CRNs is  just at its beginnings.




   Let us cite here a famous inspirational citation of Maryam Mirzakhani, to whom mathematics often felt like ``being lost in a jungle and trying to use all the knowledge that you can gather to come up with some new tricks”. It is maybe fair to say that some ME  papers which avoid symbolic  three-dimensional RH computations in favor of simplified  two-dimensional cases are leading the reader  too quickly out of the jungle. We depart here from the two dimensional tradition, by lingering a bit in the jungle. And, when we find no way out, we  make a note that an  open question remains.

Clearly, one cannot expect nowadays the bifurcation problem to be dealt with
  symbolically for many dimensions and large numbers of parameters.
   % (note that \cite{simpson2018compendium} lists 20 types of Hopf-like bifurcations already in  two- dimensional piecewise-smooth dynamical systems).
  We believe however that it is already a worthwhile effort creating  ``model Mathematica notebooks" which compute, by calling scripts in a package,  the fixed points, stability  and simple bifurcations  for  {\bf easy deterministic  mathematical epidemiology models}. Such a symbolic package %even if not indispensable for research,
  is expected to  be useful at least pedagogically,  by offering a methodic approach to the topic (and might also be useful for refereeing and spotting errors in the rather extensive ME literature). And while we are at it, the same package may be used
  for approximating the probabilities and expected times of extinction for   associated stochastic continuous time Markov chain (CTMC) models, which are defined by essentially the same input data.
  \fi

  \iffalse

  To come back to Chat Gpt, it might never have been created without
  programmers  having organized their efforts in scripts, the so called
  ``boilerplate work" (sections of code that can be included in many places without or with minimum alterations, instead of spending time and possibly making errors writing the same section multiple times). Our motivation for writing Epid was to start organizing  the ME boilerplate work, in Mathematica.
\fi

